H-MoRe: Learning Human-centric Motion Representation for Action Analysis

In this paper, we propose H-MoRe, a novel pipeline for learning precise human-centric motion representation. Our approach dynamically preserves relevant human motion while filtering out background movement. Notably, unlike previous methods relying on fully supervised learning from synthetic data, H-MoRe learns directly from real-world scenarios in a self-supervised manner, incorporating both human pose and body shape information. Inspired by kinematics, H-MoRe represents absolute and relative movements of each body point in a matrix format that captures nuanced motion details, termed world-local flows. H-MoRe offers refined insights into human motion, which can be integrated seamlessly into various action-related applications. Experimental results demonstrate that H-MoRe brings substantial improvements across various downstream tasks, including gait recognition(CL@R1: +16.01%), action recognition(Acc@1: +8.92%), and video generation(FVD: -67.07%). Additionally, H-MoRe exhibits high inference efficiency (34 fps), making it suitable for most real-time scenarios. Models and code will be released upon publication.

==> section/00_abs_v1.tex <==
\begin{abstract}

%
% NeuIPS version
%
% Action analysis is a fundamental field in computer vision, which involves the identification and interpretation of human actions from videos. Within this field, human-related motion representation plays an important role as it directly pertains to the understanding and prediction of human actions. To advance the effectiveness of these analysis tasks, this paper introduces a novel paradigm, named \textbf{H}uman-centric \textbf{Mo}tion \textbf{Re}presentation (\methodName), aimed at enriching the analytical capabilities of practical action analysis tasks. The proposed \methodName constructs a joint constraint model by integrating human motion and semantic information. Uniquely, human motion directly enhances the accuracy of human-centric motion analysis, while human semantic information supports semantically sensitive tasks such as biometric recognition. Besides, inspired by physical kinematics, we aim to integrate human-centric motion information from various coordinate systems to facilitate the learning of subsequent analysis algorithms. Consequently, we develop a dual coordinate system-based motion estimation network that efficiently infers both global motions relative to the ground and local motions relative to the individual from sequential frames. This significantly enhances the efficiency and accuracy of downstream action analysis tasks, such as gait recognition~{\small(11.09\%\(\uparrow\))}, action recognition~{\small(1.67\%\(\uparrow\))}, and video generation~{\small(59.28\%\(\uparrow\))}.

\mfinish{Oct.6}
Action analysis is a fundamental field in computer vision, which aims at analyzing complex human-related motions and extracting corresponding information. Within this field, motion estimation plays a crucial role as it directly impacts the accuracy of action sequence understanding. To further enhance the performance of human-related practical action analysis models, this paper introduces a novel learning method, named \textbf{H}uman-centric \textbf{Mo}tion \textbf{Re}presentation (\methodName{}), designed to capture richer human motion information in various scenarios. 
Leveraging biological priors from the human body, \methodName{} constructs a self-supervised learning architecture. This architecture employs a joint constraint algorithm combining skeletal dynamics with human-related geometry information to enhance motion estimation. Within these constraints, the skeleton determines the overall direction and intensity of the motion (\eg useful for video generation), while the geometric information infers the finer details of the motion (\eg beneficial for gait recognition). 
Furthermore, inspired by physical kinematics, we integrate human motion information across two distinct coordinate systems to allow the action analysis model to reason about motion from multiple perspectives, similar to how humans do. Across the two coordinate systems, one determines each point's offset between two consecutive frames relative to the world, referred to as World Motion, while the other represents each point's offset relative to the subject itself, termed Local Motion. 
% \methodName distinguishes itself by leveraging biological priors and integrating multi-coordinate system representations, providing a comprehensive approach to human motion analysis.
Leveraging these two key features, \methodName{} provides more human motion representation and significantly enhances the performance of practical action analysis models, including gait recognition~{\small(11.09\%\(\uparrow\))}, action recognition~{\small(1.67\%\(\uparrow\))}, and video generation~{\small(59.28\%\(\uparrow\))}.
\end{abstract}

==> section/00_abs_v2.tex <==
\begin{abstract}
\mfinish{Oct.20} Human-centric motion representation is an essential approach for understanding and modeling the intricate dynamics of human actions, providing crucial insights for autonomous systems across multiple domains. To enhance practical action analysis, this paper introduces a novel self-supervised learning framework, termed \methodName{}, that combines pose information and flow representation to provide an innovative and detailed understanding of human motion for practical action analysis tasks.
By leveraging multiple priors, \methodName{} constructs a Joint Constraint Learning Framework that enables learning human motion from real-world scenarios without labeled data. Besides, we introduce W-L Flows, which represent human movement from both an absolute (World Motion) and a relative (Local Motion) perspective, facilitating the capture of complex human dynamics and enhancing action analysis models across diverse tasks.
Experimental results demonstrate significant improvements in various action analysis applications, including gait recognition~{\small(11.09\%\(\uparrow\))}, action recognition~{\small(1.67\%\(\uparrow\))}, and video generation~{\small(59.28\%\(\uparrow\))}.
\end{abstract}

==> section/01_intro_v1.tex <==
\section{Introduction}

% background: human related video understanding
% -> tasks:action recognition, person re-id, video generation
% -> target: we need more accurate human motion representation
The intricate nature of human action and its broad implications have placed the understanding and representation of human actions at the forefront of computer vision research. \mold{This understanding}\mnew{Building on this foundational insight, the human motion representation} is crucial across a range of applications, from the rehabilitation~\cite{gu2019home, francisco2022computer} in healthcare to video surveillance~\cite{francisco2022computer, zhu2017flow} in security sectors. Accurate capture and interpretation of human motion are key to technological advancements across these diverse sectors. Recent developments have advanced fields such as action recognition~\cite{kar2017adascan, sun2018optical, piergiovanni2019representation}, person re-identification~\cite{zhu2021gait, cheng2017discriminative, laptev2008learning}, and video content generation~\cite{yang2023rerender, hu2023dynamic, ni2023conditional, hu2023videocontrolnet}, emphasizing the need for sophisticated human-centric motion analysis. \mold{However, the quest for an authentic and deep-seated representation of human motion, capable of navigating the complexities of real-world scenarios, remains largely unmet. This gap highlights the urgent need for new approaches capable of more effectively extracting and leveraging the intricate details of human motion.}\mnew{Although some methods developed for specific tasks integrate mechanisms for extracting motion information, seeking a unified approach that can effectively represent human motion across various vision tasks remains an important endeavor.}

% motion representations -> optical flow -> which is focus on estimating per-pixel motion between video frames
% -> more fit for Anomaly Detection (e.g. Car Accident), Sports Recognition (e.g. Ball’s Trajectory), Human-Things Interaction (e.g. Behavior Prediction).
% -> core of these optical flow's target tasks is the movement of Objects. (object-centric scenes.)
% -> human-build datasets with ground truth (Flying Chairs, Flying Things, Driving, Sintel, Monkaa, etc.)
% -> so how we analysis the scenarios of human-centric ones?
% -> cvpr 2018 PoseFlow: initial thinking about this, but constrain by the flow learning method, they use skeleton as pseudo ground truth label.
% -> total different from optical flow -> need new learning method -> kinematic semantic dual constraint learning
% -> world referenced -> self referenced
Optical Flow, the estimated of per-pixel motion between consecutive video frames~\cite{teed2020raft}, has long been the cornerstone for representing motion within the field of computer vision. 
Widely adopted in tasks ranging from anomaly detection~\cite{duman2019anomaly, liu2021hybrid}, such as in car accidents to sports recognition~\cite{mendi2013sports, tanberk2020hybrid}, like tracking a ball's trajectory, and human-object interactions~\cite{zhao2020improved, liu2020amplifying, li2020hoi}, predicting actions~\cite{bei2021learning, wu2021motionrnn}, optical flow has demonstrated remarkable utility. 
%Particularly in recent years, 
Recent advances have led to significant improvements, with algorithms excelling in object-centric scenarios. 
%Despite these advancements, 
Nevertheless, the challenge of acquiring genuine optical flow in real-world settings remains, as they are nearly impossible to capture~\cite{ilg2017flownet}. 
This limitation has led to the development of synthetic datasets, such as Flying Chairs~\cite{dosovitskiy2015flownet} and Sintel~\cite{butler2012naturalistic}, which have considerably propelled the field forward. Yet, when shifting focus to human-centric real-world scenarios, \mnew{despite relying on constraints such as photometric consistency, and smooth loss, optical flow algorithms struggle to effectively learn from those human-centric scenarios that demand high precision. This is particularly evident in tasks} such as distinguishing whether people are walking or running~\cite{de2009effects}, identifying the sports being played~\cite{wu2022survey}, or evaluating a diver's score~\cite{li2018resound}.

\citet{zhang2018poseflow} makes one of the early attempts to tackle this discrepancy by contemplating human-centric evaluation within optical flow, influenced by traditional loss functions. By constructing pseudo labels from frame-to-frame skeletal offsets and employing the standard EndPoint Error~(EPE) for flow estimation, PoseFlow presents a novel approach to embodying body skeleton-aware representation. However, %despite offering novel solutions for human-centric scenarios, 
PoseFlow remains tightly coupled with optical flow paradigms, thus inheriting constraints from its pseudo-label generation process. This association often led to the dismissal of essential human body semantic information and vulnerability to errors from skeleton estimation.

Inspired by these fantastic works, our work reevaluates the relationship between Human Motion and Optical Flow, proposing that an effective representation of human-centric motion should complement rather than conform to the constraints of optical flow paradigms. 
We advocate for a semantic-kinematic joint constraint learning method, focusing on the intrinsic information of human motion while maintaining the semantic information from original frames. 
Besides, unlike prior works that align with world-referenced offsets, our approach introduces a new pipeline that provides both world-referenced and local-referenced offsets. This novel representation has shown a superior performance in human-centric applications such as gait recognition and action recognition, marking a significant step forward in capturing the subtleties of human motion within complex real-world scenarios.

\begin{figure}[t]
  \centering
  \includegraphics[trim=0 0 0 0,clip,width=0.98\textwidth]{assets/firstview.png}
  \caption{Visualization of our HuMoR. {\small The left side of this figure shows the constrast between our proposed \textbf{Hu}man-centric \textbf{Mo}tion \textbf{R}epresentation (HuMoR) and Optical Flow. The right side displays examples of HuMoR applied to various tasks (e.g., action recognition, video generation). The color map, provided at the right-top corner, indicates motion direction and magnitude: hue represents the direction of motion, while intensity (value) reflects the magnitude of motion.}
  % The left side of this figure contrasts our proposed human-centric motion representation method (HuMoR) with optical flow. The right side shows examples of HuMoR applied to various tasks (e.g., sports analysis, video generation) across different datasets. The color map is shown at right corner.
  } 
  \label{fig:first_figure}
  \vspace{-12pt}
\end{figure}

Our contributions can be summarized as follows:
\begin{enumerate}[label=\textbf{\small(\arabic*)}, leftmargin=*]
    \item In reevaluating the relationship between optical flow and human motion analysis, our research introduces a novel form of human-centric motion representation, termed HuMoR. This representation significantly advances the field by intricately capturing human motion across dual-coordinate systems, offering a powerful modality that complements optical flow techniques.
    \item \mold{Further, we propose a pioneering self-supervised learning approach, the kinematic-semantic dual-constraint learning, which ingeniously leverages contextual kinematic information and semantic cues from images to dynamically constrain the learning process of human-centric motion representation.}\mnew{By establishing a paradigm for HuMoR and deriving such paradigm through a series of well-designed continuous functions, we ingeniously utilize semantic cues and contextual kinematic information from images to dynamically guide the self-supervised estimation of human-centric motion representation.}
    \item Empirical evidence from extensive experiments demonstrates HuMoR's superiority in enhancing the accuracy of several human-centric action analysis tasks, such as gait recognition and action recognition, beyond current related works. Moreover, in complex scene tasks, HuMoR synergistically complements Optical Flow, collectively elevating the precision of practical tasks.
\end{enumerate}

==> section/01_intro_v2.tex <==
\section{Introduction \mfinish{Oct.7}} \label{sec:introduction}

% background: human related video understanding
% -> tasks:action recognition, person re-id, video generation
% -> target: we need more accurate human motion representation

%
% NeuIPS version
%
% The intricate nature of human action and its broad implications have placed the understanding and representation of human actions at the forefront of computer vision research. Building on this foundational insight, the human motion representation is crucial across a range of applications, from the rehabilitation~\cite{gu2019home, francisco2022computer} in healthcare to video surveillance~\cite{francisco2022computer, zhu2017flow} in security sectors. Accurate capture and interpretation of human motion are key to technological advancements across these diverse sectors. Recent developments have advanced fields such as action recognition~\cite{kar2017adascan, sun2018optical, piergiovanni2019representation}, person re-identification~\cite{zhu2021gait, cheng2017discriminative, laptev2008learning}, and video content generation~\cite{yang2023rerender, hu2023dynamic, ni2023conditional, hu2023videocontrolnet}, emphasizing the need for sophisticated human-centric motion analysis. Although some methods developed for specific tasks integrate mechanisms for extracting motion information, seeking a unified approach that can effectively represent human motion across various vision tasks remains an important endeavor.

\com{YK: Overall, I feel the motivation is a bit wordy and the writing logic is not clear to me. }
Human motion, with its inherent complexity and the critical need for analysis, has established itself as a central focus in the field of computer vision. 
As a bridge to understanding and capturing the detailed dynamics of human motion, human motion representation is crucial across various practical action analysis tasks, from rehabilitation~\cite{gu2019home, francisco2022computer} in healthcare to video surveillance~\cite{francisco2022computer, zhu2017flow} in security sectors.
With rapid advancements in computer vision, increasingly complex analysis tasks, such as action recognition~\cite{kar2017adascan, sun2018optical, piergiovanni2019representation}, person re-identification~\cite{zhu2021gait, cheng2017discriminative, laptev2008learning}, and video generation~\cite{yang2023rerender, hu2023dynamic, ni2023conditional, hu2023videocontrolnet}, are becoming feasible, increasing the demand for precise motion representation in human-centric sequences.
Despite some specific action analysis models implicitly modeling motion, there remains a significant need for an explicit approach that effectively represents human motion across various practical action analysis tasks.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{asset/first_figure.pdf}
    \caption{Caption.}
    % The left side of this figure contrasts our proposed human-centric motion representation method (HuMoR) with optical flow. The right side shows examples of HuMoR applied to various tasks (e.g., sports analysis, video generation) across different datasets. The color map is shown at right corner. 
    \label{fig:first_figure}
\end{figure}

% motion representations -> optical flow -> which is focus on estimating per-pixel motion between video frames
% -> more fit for Anomaly Detection (e.g. Car Accident), Sports Recognition (e.g. Ball’s Trajectory), Human-Things Interaction (e.g. Behavior Prediction).
% -> core of these optical flow's target tasks is the movement of Objects. (object-centric scenes.)
% -> human-build datasets with ground truth (Flying Chairs, Flying Things, Driving, Sintel, Monkaa, etc.)
% -> so how we analysis the scenarios of human-centric ones?
% -> cvpr 2018 PoseFlow: initial thinking about this, but constrain by the flow learning method, they use skeleton as pseudo ground truth label.
% -> total different from optical flow -> need new learning method -> kinematic semantic dual constraint learning
% -> world referenced -> self referenced

%
% NeuIPS version
%
% Optical Flow, the estimated of per-pixel motion between consecutive video frames~\cite{teed2020raft}, has long been the cornerstone for representing motion within the field of computer vision. 
% Widely adopted in tasks ranging from anomaly detection~\cite{duman2019anomaly, liu2021hybrid}, such as in car accidents to sports recognition~\cite{mendi2013sports, tanberk2020hybrid}, like tracking a ball's trajectory, and human-object interactions~\cite{zhao2020improved, liu2020amplifying, li2020hoi}, predicting actions~\cite{bei2021learning, wu2021motionrnn}, optical flow has demonstrated remarkable utility. 
%Particularly in recent years, 
% Recent advances have led to significant improvements, with algorithms excelling in object-centric scenarios. 
%Despite these advancements, 
% Nevertheless, the challenge of acquiring genuine optical flow in real-world settings remains, as they are nearly impossible to capture~\cite{ilg2017flownet}. 
% This limitation has led to the development of synthetic datasets, such as Flying Chairs~\cite{dosovitskiy2015flownet} and Sintel~\cite{butler2012naturalistic}, which have considerably propelled the field forward. Yet, when shifting focus to human-centric real-world scenarios, despite relying on constraints such as photometric consistency, and smooth loss, optical flow algorithms struggle to effectively learn from those human-centric scenarios that demand high precision. This is particularly evident in tasks such as distinguishing whether people are walking or running~\cite{de2009effects}, identifying the sports being played~\cite{wu2022survey}, or evaluating a diver's score~\cite{li2018resound}.

\com{It seems that "human-centric" is the keyword of this work. First of all, what is our definition of human-centric and why is it better for downstream tasks? Also, 2D/3D pose can be considered as human-centric representation as its output is the pose of a person. Then what is the downside of these methods?}
To accurately represent human motion patterns, several approaches have been proposed, such as 2D pose~\cite{guler2018densepose, jiang2023rtmpose, yang2023effective}, 3D pose~\cite{zheng20213d, zhou2019hemlets, baradel2022posebert}, and Mesh~\cite{loper2023smpl, ma20233d, sun2019human, zhu2023motionbert} representations, each capable of effectively capturing the motion of the human body within a single frame. In such cases, representing human-centric motion across frames becomes especially necessary. With motion information spanning multiple frames, we can determine the speed of human motion at a given moment as well as the trends (\ie acceleration). 

\com{The transition here is not smooth. Why we care about optical flow?}
Optical flow constructs a 2D vector field to represent the offset of each pixel between consecutive frames~\cite{teed2020raft} and has been a foundational tool for motion representation in computer vision. It has been extensively used in tasks such as detecting car accidents in anomaly analysis~\cite{duman2019anomaly, liu2021hybrid}, tracking ball trajectories in sports recognition~\cite{mendi2013sports, tanberk2020hybrid}, and predicting actions~\cite{bei2021learning, wu2021motionrnn} in human-object interaction scenarios~\cite{zhao2020improved, liu2020amplifying, li2020hoi}.
However, acquiring accurate optical flow in real-world settings remains highly challenging, as ground-truth optical flow is nearly impossible to capture directly. \com{This implies that we are going to address this issue in this work.} To address this limitation, synthetic datasets such as Flying Chairs~\cite{dosovitskiy2015flownet} and Sintel~\cite{butler2012naturalistic} have been developed, significantly advancing the field. Nonetheless, when shifting focus to human-centric real-world scenarios, even with constraints such as photometric consistency and smoothness loss, existing optical flow estimation methods struggle to estimate optical flow with the precision needed to accurately represent human motion. This challenge is especially evident in tasks like distinguishing between walking and running~\cite{de2009effects}, identifying specific sports activities~\cite{wu2022survey}, or evaluating a diver's performance~\cite{li2018resound}.

\com{Up till here, I still don't know what is the challenge of learning human-centric motion representation. The challenges listed here and above are mainly for optical flow. I believe the main challenge is to learn motion that is only relevant to human body in the presence of background motion (eg leaf motion), and perhaps camera motion. One key solution is to use skeleton information to guide the learning of human-centric motion representation from flow field. }
To address these challenges, Zhang \etal. attempted to constrain optical flow estimation using skeletal information. By leveraging key points' offsets, PoseFlow~\cite{zhang2018poseflow} constructs a stick-like offset map (\cref{fig:first_figure}) as the pseudo ground truth for each frame and employs the standard optical flow estimation method (\ie Endpoint Error~(EPE)). This was an early attempt to use optical flow to represent human motion. However, due to limitations in the pseudo ground truth generation process and reliance on EPE loss, PoseFlow struggles to incorporate richer information about the human body (\eg boundaries and shape) and is highly sensitive to errors in skeleton estimation.

%
% NeuIPS version
%
% \citet{zhang2018poseflow} makes one of the early attempts to tackle this discrepancy by contemplating human-centric evaluation within optical flow, influenced by traditional loss functions. By constructing pseudo labels from frame-to-frame skeletal offsets and employing the standard EndPoint Error~(EPE) for flow estimation, PoseFlow presents a novel approach to embodying body skeleton-aware representation. However, %despite offering novel solutions for human-centric scenarios, 
% PoseFlow remains tightly coupled with optical flow paradigms, thus inheriting constraints from its pseudo-label generation process. This association often led to the dismissal of essential human body semantic information and vulnerability to errors from skeleton estimation.

In response, we propose a comprehensive human-centric motion representation that encapsulates not only motion information but also detailed body structure information based on optical flow. By leveraging the biological priors, \methodName{} constructs a self-supervised learning framework incorporating joint constraints that dynamically integrate skeletal and geometric human-related information. The skeleton-muscle constraints approximate the intensity and direction of each muscle point, while edge-chamfer constraints align the edges of the flow map with human boundaries, thereby refining the flow representation and effectively integrating detailed body information. Uniquely, inspired by physical kinematics, \methodName{} estimates human motion across two distinct coordinate systems, enabling action analysis models to reason about motion from multiple perspectives. Specifically, \methodName{} generates two types of flow maps: one captures the offset of each point between consecutive frames relative to the world, termed World Motion, while the other captures the offset relative to the subject, termed Local Motion, demonstrated in \cref{fig:first_figure}. By representing the human motion from these dual perspectives, \methodName{} significantly enriches motion representation and enhances the performance of action analysis models.

%
% NeuIPS version
%
% Inspired by these fantastic works, our work reevaluates the relationship between Human Motion and Optical Flow, proposing that an effective representation of human-centric motion should complement rather than conform to the constraints of optical flow paradigms. 
% We advocate for a semantic-kinematic joint constraint learning method, focusing on the intrinsic information of human motion while maintaining the semantic information from original frames. 
% Besides, unlike prior works that align with world-referenced offsets, our approach introduces a new pipeline that provides both world-referenced and local-referenced offsets. This novel representation has shown a superior performance in human-centric applications such as gait recognition and action recognition, marking a significant step forward in capturing the subtleties of human motion within complex real-world scenarios.

Our contributions can be summarized as follows:
\begin{enumerate}
    \item To accurately extract human-centric motion from real-world scenarios, we introduce a self-supervised learning method termed the Joint Constraint Learning Framework, enabling the estimation model to effectively learn human motion and body information from any sequence.
    \item By deeply considering the correlation between human-centric motion representation and action analysis tasks, we introduce dual flow maps under two distinct coordinate systems, termed World Motion and Local Motion. This allows \methodName{} to capture complex human motion and provide richer insights for practical action analysis tasks.
    \item Extensive experimental evidence shows \methodName{}'s superiority in enhancing the performance of various action analysis tasks, including gait recognition, action recognition, and video generation.
\end{enumerate}

%
% NeuIPS version
%
% Our contributions can be summarized as follows:
% \begin{enumerate} % [label=\textbf{\small(\arabic*)}, leftmargin=*]
    % \item In reevaluating the relationship between optical flow and human motion analysis, our research introduces a novel form of human-centric motion representation, termed HuMoR. This representation significantly advances the field by intricately capturing human motion across dual-coordinate systems, offering a powerful modality that complements optical flow techniques.
    % \item By establishing a paradigm for HuMoR and deriving such paradigm through a series of well-designed continuous functions, we ingeniously utilize semantic cues and contextual kinematic information from images to dynamically guide the self-supervised estimation of human-centric motion representation.
    % \item Empirical evidence from extensive experiments demonstrates HuMoR's superiority in enhancing the accuracy of several human-centric action analysis tasks, such as gait recognition and action recognition, beyond current related works. Moreover, in complex scene tasks, HuMoR synergistically complements Optical Flow, collectively elevating the precision of practical tasks.
% \end{enumerate}

==> section/01_intro_v3.tex <==
\section{Introduction \mfinish{Oct.20}} \label{sec:introduction}
\com{A general comment: try your best to avoid using complex and long sentences. A rule of thumb is that a sentence should be less than 4 lines. You may break a long sentence into two short ones. In addition, the first sentence of each paragraph needs to convey the key information of the paragraph.}

\com{How about we start by saying ``Understanding human motion is one of the key problems in computer vision. Using human motion, a variety of tasks can be solved, including action recognition, gait recognition, etc. However, one of the main challenges in learning human motion is to learn so-called human-centric motion, where the goal is to extract motion only from human body, while suppressing the motion information from the background. Existing methods to learning motion representation can be roughly categorized into flow-based and pose-based methods....}
Human-centric Motion Representation is a pivotal approach for modeling the intricate dynamics of human actions and plays an essential role in enabling autonomous perception systems to understand human behavior effectively. It aims to explicitly characterize diverse types of human action, capturing both their spatial and temporal features, which are crucial for a detailed understanding of human activities. Such a representation finds applications across multiple computer vision domains, including healthcare rehabilitation, video surveillance, and sports analytics, where precise modeling of human actions is fundamental. Human-centric motion representation enhances interpretability and substantially improves their predictive capabilities in complex environments, making it a cornerstone for advancing action analysis systems.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{asset/first_figure.pdf}
    \caption{Caption.}
    % The left side of this figure contrasts our proposed human-centric motion representation method (HuMoR) with optical flow. The right side shows examples of HuMoR applied to various tasks (e.g., sports analysis, video generation) across different datasets. The color map is shown at right corner. 
    \label{fig:first_figure}
\end{figure}

\com{I expect to see what are the challenges in learning human-centric motion representation and how existing methods are address the challenges.}
Early works such as TSN~\cite{} and I3D~\cite{} attempted to model temporal information by employing deep neural networks~(DNNs) to implicitly learn motion features from video sequences. However, due to the inherent complexity of human actions, these implicit modeling approaches often struggle to accurately capture the fine-grained dynamics required for tasks that demand precise discrimination, \eg gait recognition~\cite{}. Consequently, research attention has shifted towards explicitly representing these motions \com{references are needed to support this claim}. Explicit human-centric motion representation relies on two critical parts: the representation carriers and the learning strategies \com{I would remove this sentence because you did not categorize methods according to their learning methods}. These components determine how effectively human motion can be represented for subsequent analysis and applied to complex scenarios.


\com{How about move this paragraph to the second paragraph so that it would be clear to see existing methods for learning motion representation?} Two primary carriers for motion representation are Flow-based methods and Pose-based methods. Flow-based methods, such as optical flow, create dense 2D vector fields that encode pixel offsets between consecutive frames, thereby capturing inter-frame motion information, including speed (slow or fast), acceleration trends, \etc. In contrast, pose-based methods focus on capturing the position and shape of the human body in each frame, thus providing substantial information about the human shape and posture within single frames \com{I still have doubts for the pose-based methods. Is it right to claim them as learning motion representation? How can motion be learned from a single frame?}.

\com{Again, I am not clear that why we need such a long paragraph to describe the limitations of flow-based approaches. You need to only focus on 1-2 pieces of this category to better motivate your work.}
Flow-based approaches establish significant temporal representations of motion. However, their performance is constrained by synthetic datasets like FlyingChairs and FlyingThings~\cite{}, making it difficult to effectively learn human-related information in real-world environments \com{I don't think this statement is true. There are tons of flow-based methods, such as TSN, that have been applied to real data}. As a result, these methods often struggle in human-centric scenarios (\eg sports analysis~\cite{}) compared to object-centric contexts (\eg traffic accident detection~\cite{}) \com{They struggle because they don't really know where the humans are and thus the motion contains both human motion and background motion}. On the other hand, pose-based methods, which inherently focus on human-centric features \com{Again, we need to carefully define what is "human-centric"}, primarily capture information at a single-frame level and therefore require subsequent temporal modeling algorithms, \eg ST-GCN~\cite{}, to establish temporal and spatial representations. This reliance on additional temporal modeling necessitates specialized architectures that can effectively leverage this information, unlike flow-based methods which can be integrated non-invasively. With the rise of large-scale models, such as ViTs~\cite{} serving as large-scale encoders, leveraging pose-based information has become increasingly challenging, as these models favor global features learned from multi-modality inputs instead of temporal modeling based on graph architectures.


PoseFlow~\cite{} emerged as an attempt to synergize these two carriers by fusing pose-based skeletal dynamics with flow-based motion representations, thereby aiming to construct a richer, more informative depiction of human actions. In PoseFlow, keypoint offsets are used to generate pseudo ground truth for the flow estimation process. Despite its innovative fusion approaches, PoseFlow's dependency on handcrafted pseudo ground truth and its reliance on Endpoint Error~(EPE) loss present significant limitations. Specifically, PoseFlow lacks the ability to effectively incorporate detailed body boundary information, and it is highly susceptible to inaccuracies in skeleton estimation. Consequently, its capacity to robustly represent complex, real-world human-centric motion remains constrained.

\com{Our goal is not to address the limitation of PoseFlow and not to improve it. Our goal is to address the challenges if learning human-centric motion representation. }
To address the limitations inherent in PoseFlow, as well as the second critical aspect of explicit human-centric motion representation, we propose a novel learning framework, termed \methodName{} (Human-More). \methodName{} is designed to effectively learn human-centric motion representation by integrating pose information and flow-based representation with detailed geometric information. Our approach leverages multiple priors about the human body to guide the representation learning process by constructing a self-supervised learning framework, enabling nuanced and robust human-centric motion representations without relying heavily on either synthetic or labeled datasets. This refined representation captures the benefits of both flow-based and pose-based methods, leading to a more comprehensive understanding of human dynamics. \com{This paragraph suppose to write how the proposed method addresses the key challenges of learning human-centric motion. All the description should be centered around the solutions to challenges. I don't see it in this paragraph.}

Specifically, our framework introduces two distinct motion representations: World Flow and Local Flow, collectively termed W-L Flows. World Flow characterizes the movement of the human body relative to the world, effectively capturing absolute positional dynamics, while Local Flow represents movement relative to the subject's own body, emphasizing intrinsic motion details. This dual-perspective approach allows for more nuanced modeling of human-centric motion by capturing both absolute and relative dynamics.

To facilitate the learning of W-L Flows from diverse real-world scenarios, we introduce the Joint Constraint Learning Framework, which consists of the Skeleton-Body Constraint and the Boundaries-Edge Constraint. The combined influence of these two constraints enables the flow to infer the approximate movement range of different body points based on skeletal information, and subsequently refine this range using human boundary details.

Building on previous wonderful works in pose-based and flow-based representation, \methodName{} surpasses the limitations of existing human-centric motion representation approaches. This leads to a more sophisticated and interpretable representation of human-centric motion, significantly improving the accuracy of motion depiction. Consequently, \methodName{} enhances the performance of action analysis models, delivering superior results across a range of real-world scenarios that require detailed understanding and prediction of human actions.

Our contributions can be summarized as follows:
\begin{enumerate}
    \item To accurately extract human-centric motion from real-world scenarios, we introduce a self-supervised learning method termed the Joint Constraint Learning Framework, enabling the estimation model to effectively learn human motion and body information from any sequence.
    \item By deeply considering the correlation between human-centric motion representation and action analysis tasks, we introduce dual flow maps under two distinct coordinate systems, termed World Motion and Local Motion. This allows \methodName{} to capture complex human motion and provide richer insights for practical action analysis tasks.
    \item Extensive experimental evidence shows \methodName{}'s superiority in enhancing the performance of various action analysis tasks, including gait recognition, action recognition, and video generation.
\end{enumerate}

==> section/01_intro_v4.tex <==
\section{Introduction {\small \mfinish{Nov.8} \TODO{Updating}}} \label{sec:introduction}

Understanding human motion has long been a fundamental challenge in computer vision.
By leveraging motion information, numerous practical vision tasks can be tackled, from rehabilitation~\cite{} in healthcare to video surveillance~\cite{} in security sectors. These analyses are completed by recognizing patterns in human motion information rather than the motion of irrelevant background elements, \eg tree leaves. Thus, to further boost analysis performance, we need to provide precise motion highly relevant to humans, \ie, human-centric motion.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{asset/first_figure.pdf}
    \caption{Illustration of Existing Motion Representations: Including single-frame pose information and cross-frame optical flow. Our approach introduces a novel flow representation to capture human motion across frames.}
    \label{fig:first_figure}
\end{figure}

Currently, two widely used motion representations are optical flow and human pose.
% optical flow
Optical flow captures motion between consecutive frames by utilizing a flow map to represent offsets for each pixel. Due to the feature of the flow map, \ie matrix, it encodes both motion and shape information, as well as can be easily integrated into convolutional neural networks (CNNs) or vision transformers (ViTs). Thus make it a popular choice for action recognition~\cite{} and video generation~\cite{}.
However, it calculates offsets indiscriminately for all pixels, making it inadequate for human-centric requirements. Additionally, learning from synthetic datasets leaves it lacking the knowledge needed to capture nuanced human motion.
% pose information
Hence, in recent years, many analysis tasks instead obtain human-centric motion from pose information. They utilize graph neural networks (GNNs) to extract spatial-temporal features from pose information from each frame.
Pose information, as it contains only skeletal points in 2D~\cite{} or 3D~\cite{} coordinates, provides pure human-centric information. However, it lacks shape information, which is particularly important for numerous analysis tasks, \eg body shape for gait recognition~\cite{}.



% Currently, two widely used methods for motion representation in the field of action analysis are optical flow and human pose. 
% Optical flow captures inter-frame motion by representing pixel offsets between consecutive frames, effectively encoding motion and object shape information. 
% Due to its matrix representation, optical flow can be easily processed and learned by convolutional neural networks (CNNs) and vision transformers (ViTs), which makes it a popular choice for action recognition~\cite{} as well as a condition for video generation~\cite{}. 
% However, its reliance on learning from synthetic datasets~\cite{} limits its performance to predominantly object-centric scenarios (\eg traffic accident~\cite{}), rendering it less effective in capturing nuanced human motion. Hence, in recent years, many human pose estimation approaches~\cite{} have gained prominence. 
% These methods estimate skeletal keypoints in 2D~\cite{} or 3D~\cite{} in each frame, which, when combined with graph neural networks (GNNs) like ST-GCN~\cite{}, enable detailed analysis of human motion. This approach provides accurate human-centric motion information that greatly benefits practical action analysis systems. However, human pose are heavily dependent on specialized network architectures, making it less adaptable as an auxiliary modality to be easily integrated with other modalities in large-scale action-related models (\eg in video generation~\cite{}).

To address these challenges, we propose a new human-centric motion representation that aims to retain both precise human motion and shape information while being seamlessly integrable into action-related systems. Specifically, our novel flow map, termed \methodName{}, is designed to encapsulate the accurate human pose while maintaining the usability and interpretability of optical flow.

To effectively learn \methodName{} from real-world scenarios, we design a Joint Constraint learning framework, including skeleton-body and boundary-edge constraints. 
Unlike optical flow, which relies on supervised learning (\eg EndPoint Error~\cite{}) from synthetic datasets designed for object-centric scenarios, we incorporate precise human motion information by using skeleton-body constraints derived from the human pose. 
Specifically, by using skeletal offsets to constrain the estimated flow for each body points, we ensure \methodName{} provides an accurate representation of human motion. 
Additionally, unlike human pose representations that rely solely on keypoints, the flow representation allows us to introduce body shape information into \methodName{}. By aligning the edges in the flow map with human boundaries through the boundaries-edge constraint, we refine the details of human motion, such as hand movements, while incorporating overall body shape information. This enriched representation enhances the performance of action analysis tasks that require both motion and shape information, such as gait recognition~\cite{} and video generation~\cite{}.

Similar to the consensus in using GNNs for analyzing human pose, capturing underlying motion information is crucial for effective action analysis. Inspired by physical kinematics, \methodName{} introduces W-L Flows, consisting of World Flow and Local Flow. World Flow captures each body point's offset relative to the external environment, \eg the ground or camera, effectively encoding absolute positional dynamics, while Local Flow represents offsets relative to the subject's own body, emphasizing intrinsic motion details. This dual-perspective approach allows for a more comprehensive and nuanced modeling of human motion, capturing both absolute and relative motions to enhance tasks that require precise analysis of motion, \eg diving analysis in aquatics championships~\cite{}.

Our contributions can be summarized as follows:
\begin{enumerate}
    \item To provide a human-centric motion representation with accurate human motion like human pose while maintaining usability and interoperability like optical flow, we introduce an innovative flow map termed \methodName{}.
    \item To accurately extract \methodName{} from real-world scenarios, we introduce the Joint Constraint learning framework, enabling the estimation model to effectively learn human motion from any sequence without ground truth like optical flow estimation algorithms.
    \item To capture underlying motion information for effective action analysis, we propose W-L Flows, which enable us to capture both absolute and relative motions and provide richer insights about human motion for practical action analysis models.
    \item Extensive experimental evidence shows \methodName{}'s superiority in enhancing the performance of various action analysis tasks, including gait recognition, action recognition, and video generation.
\end{enumerate}


==> section/02_related_v1.tex <==
\section{Related Work {\small \mfinish{Oct.7} \TODO{Need Update}}} \label{sec:related_work}

% optical flow -> genric / object related scenarios analysis
% new representation method -> human-centric scenarios analysis

%
% NeuIPS version
%
% In practical vision tasks, modalities for characterizing motion are crucial. This section reviews developments in optical flow for object-centric applications and pose-based human motion estimation for human-centric contexts, highlighting their importance in analyzing real-world scenarios.

Motion information across frames (\ie flow) is crucial for practical action analysis tasks as it captures both the velocity and acceleration of motion. This section reviews object-centric optical flow estimation algorithms and the evolution of methods that utilize pose information to guide or refine optical flow estimation, highlighting their significance for analyzing real-world scenarios.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{asset/problem_formulation.pdf}
%   \caption{}
%   \label{fig:problem_formulation}
% \end{figure*}

\paragraph{Object-centric Optical Flow Estimation}
% initial of optical flow -> minimization problem -> motion detection & tracking
% cnns -> flownet -> dataset (pseudo label) & loss (learning paradigms) -> [foreshadowing: diff from optical paradigms]
% raft -> recurrent
% transformer -> well designed encoder & decoder

%
% NeuIPS version
%
% Originally, the optical flow was conceived as an energy minimization problem, was pioneered by \citet{horn1981determining}, leveraging brightness constancy and spatial smoothness principles. Initially, optical flow was employed to address challenges such as motion detection and tracking in less complex settings, providing a foundational understanding of pixel movements between consecutive frames. With the rapid evolution of Convolutional Neural Networks (CNNs) sparked a revolution in optical flow estimation. FlowNet\cite{dosovitskiy2015flownet} emerged as a landmark work, pioneering the end-to-end learning approach by directly regressing optical flow from consecutive image pairs. This model, utilizing techniques such as stacked network architectures and iterative refinement, laid the groundwork for future research by establishing the FlyingChairs dataset. This dataset, crafted through computer-simulated motion, set a precedent for generating frame-by-frame ground truth optical flows~\cite{ilg2018occlusions, ilg2017flownet, mayer2016large, butler2012naturalistic, menze2015object, kondermann2016hci, sun2022disentangling}, promoting a regression-based learning model employing loss functions like Mean Absolute Error (MAE) and Mean Squared Error (MSE). The introduction of such datasets marked a significant advancement, facilitating a surge in deep learning-based optical flow methodologies. Inspired by the coarse-to-fine strategies, RAFT~\cite{sui2022craft} was introduced, representing a paradigm shift in optical flow estimation. By iteratively refining flow predictions and employing all-pairs field transforms, RAFT significantly enhanced the accuracy of capturing minute motions, setting a new standard for the precision of optical flow estimations. This innovative approach fueled a series of distinct subsequent works, such as CRAFT~\cite{sui2022craft} and GMA~\cite{jiang2021learning}, each introducing unique elements to the iterative refinement process and further advancing the field. Recently, the advent of Transformer-based methodologies has redefined optical flow estimation. Techniques such as GMFlow~\cite{xu2022gmflow}, which addresses optical flow as a matching problem, and architectures like FlowFormer~\cite{huang2022flowformer} and FlowFormer++~\cite{shi2023flowformer++} that optimize Transformer capabilities through cost encoding and Masked Cost-Volume Autoencoding, have showcased exceptional improvements in accuracy and robustness, particularly in adverse conditions. These developments not only illustrate the continuous evolution of optical flow estimation but also highlight the increasing complexity and precision in understanding pixel dynamics across diverse environments.
% Originally, the optical flow is framed as an energy minimization problem by~\citet{horn1981determining}, applied principles of brightness constancy and spatial smoothness to facilitate motion detection and tracking.
% The onset of deep learning, particularly with FlowNet~\cite{dosovitskiy2015flownet}'s introduction, marks a significant shift, pioneering end-to-end optical flow learning via CNNs. 
% This shift is accompanied by the development of synthetic datasets like FlyingChairs~\cite{ilg2018occlusions, ilg2017flownet, mayer2016large, butler2012naturalistic, menze2015object, kondermann2016hci, sun2022disentangling}, which, by simulating motion, establish a new standard for generating ground truth data and adopting regression-based models using losses like MAE and MSE. 
% Building on coarse-to-fine approaches, RAFT~\cite{sui2022craft} introduces an innovative iterative refinement technique, significantly enhancing micro-motion accuracy and setting new standards for flow estimation. 
% This spurs a range of methodologies, such as CRAFT~\cite{sui2022craft} and GMA~\cite{jiang2021learning}, advancing iterative refinement in flow computation. 
% Recently, Transformer-based methods further evolves optical flow estimation. 
% Innovations such as GMFlow~\cite{xu2022gmflow} and architectures like FlowFormer~\cite{huang2022flowformer} and FlowFormer{\scriptsize++}~\cite{shi2023flowformer++} have demonstrated significant accuracy and robustness improvements, especially under challenging conditions. These advancements underscore the field's progression towards more intricate and precise motion understanding.

Originally, optical flow estimation was formulated as an energy minimization problem~\cite{horn1981determining}, applying the principles of brightness constancy and spatial smoothness to facilitate motion detection and tracking. The advent of deep learning, particularly with the introduction of FlowNet~\cite{dosovitskiy2015flownet}, marked a significant shift, pioneering end-to-end optical flow estimation using convolutional neural networks (CNNs). 
This transition was further supported by the synthetic datasets like FlyingChairs~\cite{ilg2018occlusions, ilg2017flownet, mayer2016large, butler2012naturalistic, menze2015object, kondermann2016hci, sun2022disentangling}, which established a new framework for generating artificial ground truth through simulation, thereby enabling regression-based flow estimation using losses such as Mean Absolute Error~(MAE) and Mean Squared Error~(MSE). 
Building on coarse-to-fine approaches, RAFT~\cite{sui2022craft} (\cref{fig:first_figure}) introduced an innovative iterative refinement technique, significantly enhancing micro-motion accuracy and setting a new benchmark for optical flow estimation. 
This advancement paved the way for a range of new algorithms, including CRAFT~\cite{sui2022craft} and GMA~\cite{jiang2021learning}, which pushed iterative refinement in the estimation process further. 
More recently, Transformer-based methods have driven the evolution of optical flow estimation. %, leveraging the powerful learning capabilities of Transformers. 
Innovations such as GMFlow~\cite{xu2022gmflow} and architectures like FlowFormer~\cite{huang2022flowformer} and FlowFormer{\scriptsize++}~\cite{shi2023flowformer++} have demonstrated significant improvements in accuracy and robustness, particularly under challenging conditions. 
These advancements underscore the progression of object-centric optical flow estimation towards greater complexity and precision.

\paragraph{Pose-guided Optical Flow Estimation}
% intro -> background -> human action analysis become more important
% poseflow -> first use pose to guide
% arko et al -> bootstrapping pose estimation & flow estimation
% they work better on human-centric scenarios
% however -> drop semantic detail -> hurt accuracy of human motion analysis
% our target -> find representation with semantic & kinematic

%
% NeuIPS version
%
% As video recognition tasks become increasingly nuanced, the significance of accurately identifying human actions has come to the forefront, as well as the generic object flow. In this context, PoseFlow~\cite{zhang2018poseflow} emerged, leveraging frame-to-frame skeletal offsets to create pseudo offset labels. This approach, illustrated in their pseudo ground truth flow maps resembling matchstick figures (seen in Fig.~\ref{fig:first_figure}), uses conventional optical flow loss metrics such as Endpoint Error for model training. Recently, \citet{arko2022bootstrapping} takes a step further by mutually correcting skeletal structures and flow maps estimated by networks. Their method, reminiscent of PoseFlow's approach, overlays the skeletal flow map onto the estimated flow map to adjust optical flow outcomes based on pose estimation results. Validating the presence of flow at skeletal points enables zero-shot adjustment of flow predictions; likewise, they enforce that the movement of 3D joints, when projected onto 2D images, aligns with the optical flow estimates. This mutual correction between pose and flow marks a significant advance in pose-guided flow estimation. However, these methodologies, heavily influenced by the field of optical flow, primarily aim to substitute or optimize flow algorithms using skeletal offsets as ground truth, at the expense of losing some semantic information. This compromise can significantly impact the accuracy of practical vision tasks, especially those requiring precise human motion recognition. With the rapid advancement in optical flow research providing accurate representations of object and environmental movement, it becomes crucial to find a representation that retains semantic integrity while accurately depicting human motion. Our work builds upon these insights, seeking a representation that maintains semantic information for precise human activity analysis. Such a representation proves effective in tasks requiring high-precision human behavior analysis, such as biometric identification and motion analytics, and complements the perception of the scenarios with the rich contextual information provided by optical flow in complex scene analysis.
% As video recognition tasks become increasingly nuanced, accurately identifying human actions alongside generic object flow has emerged as a critical challenge. 
% In this context, PoseFlow~\cite{zhang2018poseflow} emerges, leveraging frame-to-frame skeletal offsets to create pseudo offset labels. 
% This approach is illustrated by pseudo ground truth flow maps resembling matchstick figures 
% %(Fig.~\ref{fig:first_figure}) 
% and employs conventional flow loss metrics, such as EPE, for model training. Similarly, \citet{arko2022bootstrapping} advances this concept by mutually correcting skeletal structures and flow maps. 
% Their method overlays the skeletal flow map onto the estimated flow, enabling zero-shot adjustment based on skeletal alignments and ensuring 3D joint movements align with flow estimates in 2D projections. 
% This mutual correction between pose and flow marks a significant advance in pose-guided flow estimation.
% However, while these methodologies significantly advance pose-guided flow estimation, they may sacrifice semantic detail by primarily focusing on skeletal offsets as a proxy for true flow. 
% This could undermine the accuracy of tasks requiring nuanced human motion analysis. 
% In contrast, our work addresses this issue by maintaining semantic integrity within a new representation method, thereby enhancing the precision of human-centric analysis in complex environments.

As action analysis becomes increasingly refined, accurately identifying human actions from object-centric optical flow has become a critical challenge. In this context, PoseFlow~\cite{zhang2018poseflow} emerged as a method leveraging keypoint offsets between frames to construct a pseudo ground truth similar to stick-like figures (\cref{fig:first_figure}), training the optical flow estimation model using classical regression methods (e.g., Endpoint Error (EPE) loss). Similarly, Arko \etal~\cite{arko2022bootstrapping} stacked these keypoint offsets on object-centric optical flow, enabling zero-shot adjustments based on skeletal alignments and ensuring 3D keypoint movements align with fine-grained optical flow in 2D projections. This mutual correction between pose and optical flow marks a significant advancement in pose-guided optical flow estimation. However, despite these improvements in flow accuracy for human motion, these methods are still unable to preserve detailed human body information due to their reliance on keypoint offsets, which can undermine tasks requiring fine analysis of human shape and patterns. In contrast, we propose a joint constraint learning framework that dynamically binds skeletal and muscle points, employing human boundaries and a well-designed chamfer distance-based constraint to precisely align the edges of the estimated flow, thus achieving human-centric optical flow estimation and enhancing the precision of action analysis in complex environments.

==> section/03_method_v1.tex <==
\section{Methodology \mfinish{Oct.11-14} {\small \TODO{Ready for Comment}}}

%\mold{We introduce a novel paradigm for practical motion analysis, Human Motion Representation (HuMoR), designed to capture rich semantic and kinematic information to articulate human motion precisely.} \mnew{To more accurately extract motion representations for human-related action analysis tasks, we define a new approach termed Human-centric Motion Representation (HuMoR). This method captures precise human motion while incorporating substantial semantic information.} This addresses the limitations of optical flow, a widely used action analysis representation that often fails to accurately capture the subtleties of human motion within complex real-world scenarios.

%
% NeuIPS version
%
% This section is structured as follows: Sec.~\ref{sec:problem_formulation} outlines the problem formulation, laying the groundwork for our proposed HuMoR. Sec.~\ref{sec:dual_constraint} \mold{delves into the implementation details of our approach}\mnew{derives such formulation through a series of well-designed functions}, highlighting the joint constraints that underpin our representation. Lastly, Sec.~\ref{sec:network_architecture} provides an overview of the network architecture we employ to estimate human motion.

This section begins with our problem formulation, detailing how \methodName{} constructs a self-supervised learning framework and the theoretical foundation of the proposed dual-coordinate flow maps. We then further discuss how we convert these discrete constraints into differentiable matrix operations. Finally, we discuss how neural networks are used to solve our formulation.\com{Redundent. Delete this.}

\subsection{Problem Formulation {\footnotesize \mfinish{Oct.11}}} \label{sec:problem_formulation}

% overall bilevel for representation & practical vision tasks
% -> f + g_s + g_k
% -> u_w = u_l + m
% -> 2d or 3d -> show example on 2d

% We start by defining a novel paradigm for practical motion analysis tasks. Assuming the frame at time \(t\) and the motion representation are denoted as column vectors \(\boldsymbol{x_{t}}\) and \(\boldsymbol{u}\), respectively. Drawing inspiration from Stackelberg's theory, we propose that the motion representation for human-centric action analysis should adhere to the following paradigm:
% \begin{gather}
%     \min_{\boldsymbol{u ^{*}}} \mathcal{L}^{p}\left ( \Psi \left ( \boldsymbol{u ^{*}}, \boldsymbol{v} \right )  \right ), \\
%     \mathit{s.t.} ~\ \boldsymbol{u^{*}} = \argmin_{\boldsymbol{u}} f\left ( \boldsymbol{u}; \boldsymbol{x_{t}}, \boldsymbol{x_{t+1}} \right ) + g_{s}\left ( \boldsymbol{u}; \boldsymbol{x_{t}} \right ) + g_{k}\left ( \boldsymbol{u}; \boldsymbol{x_{t} \rightarrow x_{t+1}}  \right ),
%     \label{eq:problem_formulation}
% \end{gather}
% where \(\mathcal{L}^{p}\) is the analysis-specific task loss, and \(\Psi\) denotes an action analysis network that also takes other modality inputs \(\boldsymbol{v}\). \(f\left( \cdot \right)\) represents an energy-based fidelity term that includes the motion representation \(\boldsymbol{u}\), and source frames \(\boldsymbol{x_{t}}\) and \(\boldsymbol{x_{t+1}}\), while \(g_{s}\) and \(g_{k}\) serve as feasibility constraints based on the semantic and kinematic information, respectively.

%
% NeuIPS version
%
% We begin by examining the paradigm for practical action analysis tasks, as visually represented in Fig.~\ref{fig:problem_formulation}. Assuming that \(\Psi\) denotes a specific algorithm designed for action analysis, 
% with inputs that include any motion representation \(\boldsymbol{u}\) and additional modalities \(\boldsymbol{v}\) such as frames or tokens, our goal, under the premise that \(\boldsymbol{v}\) remains constant, is to precisely define a method of human motion representation named HuMoR \(\boldsymbol{u^{*}} \in \boldsymbol{u}\).
% This representation is depicted as white spheres in the figure, designed to minimizes the task-specific loss \(\mathcal{L}^{p}\), which interacts with multiple saddle surfaces. This conceptual approach is mathematically formulated as follows:
% \begin{equation}
%     \min_{\boldsymbol{u}} \mathcal{L}^{p}\left ( \Psi \left ( \boldsymbol{u}, \boldsymbol{v} \right )  \right ),
%     \label{eq:analysis_paradigm}
% \end{equation}
% where the motion representation \(\boldsymbol{u}\) may appear in various forms. 
% A common one is Optical Flow (\(\boldsymbol{u}^\mathsf{opt} \in \boldsymbol{u}\)), capturing the motion between adjacent frames \(\boldsymbol{x}_{t}\) and \(\boldsymbol{x}_{t+1}\). Inspired by such implementations, we employ frame-based functions \(f\left ( \cdot \right )\) to estimate human-centric motion \(\boldsymbol{u^{*}}\). 
% Unlike \(\boldsymbol{u}^\mathsf{opt}\), which is applicable to any object movement, our method, designed with a human-oriented perspective, specifically targets human elements. 
% Drawing inspiration from~\cite{arko2022bootstrapping, zhang2018poseflow}, we introduce an energy-based fidelity term concerning kinematics, \(g_{k}\), the brown line on sphere in figure,\mold{which leverages human priors to ensure the precision of the human motion presentation.}\mnew{which leverages biomechanical priors, ensuring that the modeled human motion adheres to realistic physiological constraints such as the alignment of muscular movements with skeletal motions.}
% Further, we incorporate a semantic term, $g_{s}$, the green line on sphere in figure, to maintain the semantic information pertinent to human subjects. Therefore, the estimation process for \(\boldsymbol{u^{*}}\) can be detailed as:
% \begin{equation}
%     \boldsymbol{u^{*}} = \argmin_{\boldsymbol{u}} f\left ( \boldsymbol{u}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + g_{s}\left ( \boldsymbol{u}; \boldsymbol{x}_{t} \right ) + g_{k}\left ( \boldsymbol{u}; \boldsymbol{x}_{t} \rightarrow \boldsymbol{x}_{t+1}  \right ).
%     \label{eq:problem_formulation}
% \end{equation}
% Fig.~\ref{fig:problem_formulation} illustrates how Eq.~\ref{eq:problem_formulation} facilitates efficient solutions for human-centric action analysis tasks.

% Furthermore, analogous to the Galilean transformation~\cite{galilei2002discourses} of kinematic analysis in classical mechanics, the judicious application of reference frame transformations significantly enhances the efficiency and accuracy of the analysis. Consequently, we decompose the \(\boldsymbol{u^{*}}\) into two components: the motion of the target relative to the world coordinate origin, denoted by \(\boldsymbol{u^{w}}\), and the motion of the target's parts relative to itself, denoted by \(\boldsymbol{u^{l}}\). According to the vector calculus theory, the relationship between \(\boldsymbol{u^{w}}\) and \(\boldsymbol{u^{l}}\) facilitates their transformation and is governed by the following equation:
% \begin{equation}
%     \boldsymbol{u^{w}} = \boldsymbol{u^{l}} + \boldsymbol{m}, \mathit{s.t.} ~\ \boldsymbol{u^{*}} = \left \{ \boldsymbol{u^{w}}, \boldsymbol{u^{l}} \right \},
%     \label{eq:multi_coordinate}
% \end{equation}
% where the \(\boldsymbol{m}\) denotes the motion vector of the target. The proposed representation encompasses a diverse range of modalities. Specifically, for a video frame of dimensions \(h \times w\), the \(\boldsymbol{u^{*}}\) is mapped onto \(\mathbb{R}^{2 \times hw \times d}\), assuming \(d=2\) to facilitate the formulation throughout this paper. Each pixel within this space encapsulates the displacement along the respective axis.
%  \mnew{In the subsequent sections, we detail the practical expansion of this formulation (Sec.~\ref{sec:dual_constraint}), demonstrating an implementation for estimating multi-coordinate origin 2D offset maps, derived from Eq.~\ref{eq:problem_formulation} in Sec.~\ref{sec:network_architecture}.}
\com{One sentence about the overall goal is missing here. We need to state that the goal is to learn human-centric motion representation by extracting human motion from noisy optical flow using human pose as a prior.}

We begin with the optical flow estimation paradigm. For a given pair of consecutive frames \( \left( \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) \) and a flow estimation function or network \com{just say this is a network} \( \Phi \), the estimated optical flow can be represented as \( \boldsymbol{u} = \Phi \left( \omega_{1}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) \) \com{Usually, parameter goes after variables}, where \( \omega_{1} \) represents variables or parameters \com{this is definitely parameters, not variables} in the function or network \com{again, just say this is a network}. For most of the existing optical flow estimation methods learning from ground truth \( \hat{\boldsymbol{u}} \), their constraints can be expressed as:\com{this meta loss can be an in-line one as it does not give new information}
\begin{equation}
    \boldsymbol{u_o} =  \arg\min_{\boldsymbol{u}}\mathcal{H}\left( \boldsymbol{u}, \hat{\boldsymbol{u}} \right), \label{eq:supervised_learning}
\end{equation}
where \(\mathcal{H}\) is typically an \( \left \| \cdot  \right \| _{n} \) \com{what is this?} applied over one or multiple scales, to ensure \( \boldsymbol{u} \) regresses towards the ground truth \( \hat{\boldsymbol{u}} \). \com{Do we really need the above equation? First, this is misleading as our method does not have supervision for optical flow. Using $\hat{u}$ confuses reviewers. Second, this is a well acknowledged definition of optical flow and we don't need to discuss this again unless new knowledge is being presented.}

\com{this is an extremely long sentence spanning over six lines} To accurately capture human motion information in real-world scenarios without ground truth, \methodName{} introduces kinematic fidelity terms, namely Skeleton-Muscule Constraint (\( \mathcal{F} \)) \com{where is this constraint defined?}, which leverage biological priors, ensuring that the movement of each muscle point adheres to realistic physiological constraints, \eg the coordination between muscle and skeletal movements. Additionally, to preserve human shape information and achieve a more precise flow map, we introduce Edge-Chamfer Constraint (\( \mathcal{G} \)) \com{where is this constraint defined?} to align the edges of the estimated flow map with human boundaries. These edges are defined by intensity and angle discontinuities, which can also be used to delineate the separation between the moving foreground and the static background. Therefore, instead of \cref{eq:supervised_learning}, our Joint Constraint Learning Framework can be represented as:
\begin{equation}
    \boldsymbol{u_w} =  \arg\min_{\boldsymbol{u}}\left [ \mathcal{F}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + \alpha \cdot \mathcal{G}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right ) \right ], \label{eq:world_constraint}
\end{equation}
where \( \boldsymbol{u_w} \) represents the World Motion estimated by our \methodName{}, and \( \alpha \) is a weight used for a trade-off.

To further advance practical action analysis models toward world models, we draw inspiration from physical kinematics and introduce a concept similar to Galilean Transformation~\cite{galilei2002discourses} in \methodName{}, namely W-L \com{what is W-L} Flows. Similar to the human beings process of analyzing motion, evaluating motion across multiple reference systems significantly improves the accuracy of conclusions. Therefore, the proposed W-L Flows include two types of motion information under two distinct coordinate systems: World Motion, which represents the true offset of each point relative to the ground (just as classical optical flow estimation algorithms do), and Local Motion, which represents the relative offset of each point with respect to the moving subject itself. This relative flow is highly beneficial for fine-grained motion analysis. According to the principles of vector decomposition, World Motion \( \boldsymbol{u_w} \) can be decomposed into Local Motion \( \boldsymbol{u_l} \) and Subject Motion \( \boldsymbol{u_s} \), where \( \boldsymbol{u_s} \) represents the true offset of the subject as a whole relative to the ground. In this progress, we can calculate \( \boldsymbol{u_l} \) by estimating \( \boldsymbol{u_w} \) and \( \boldsymbol{u_s} \), denoted as:
\begin{equation}
    \begin{gathered}
        \boldsymbol{u_w} = \boldsymbol{u_l} + \boldsymbol{u_s}, \\
        \boldsymbol{u_s} = \Psi \left( \omega_{2}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}, \boldsymbol{u_w} \right),
    \end{gathered}
    \label{eq:dual_coord_flow}
\end{equation}
where the \( \Psi \) denotes the function used to estimate \( \boldsymbol{u_s} \) based on frames and \( \boldsymbol{u_w} \), \( \omega_{2} \) represents the learnable parameters in \( \Psi \). We can theoretically obtain \( \boldsymbol{u_l} \) by this system of equations.
\com{It is not clear to me how W-L is used and linked to the objective function Eq. 2.}

%
% NeuIPS version
%
% \subsection{Semantic~-~Kinematic Joint Constraint Learning} \label{sec:dual_constraint}

% In this section, we detail a 2D implementation of the joint constraints specified in Eq.~\ref{eq:problem_formulation}. 
% Briefly, for the semantic constraint \(g_{s}\), we introduce a differentiable geometrically metric designed to align the edges of the \(\boldsymbol{u^{*}}\) with those of the frame \(\boldsymbol{x}_{t}\). 
% Meanwhile, the kinematic constraint \(g_{k}\) is realized via a dynamic constraint mechanism based on skeletal motion vectors.

% \paragraph{Semantic Constraint with Patch Centroid Distance:} Semantic information, particularly human body edge information, plays a pivotal role in human motion analysis~\cite{tseng2023edge, chai2022lagrange, pham2022video}. 
% For instance, it enhances the precision of feature extraction by locating and identifying human postures and actions accurately. 
% In the realm of 3D reconstruction, edge information assists in more accurately estimating the body structure~\cite{ye2023nef, schmied2023r3d3}. 
% Additionally, in scenarios with complex backgrounds and multiple individuals, body edge information aids in distinguishing between different people~\cite{he2020bdcn}. 
% Given these considerations, this study employs human body edge constraints to impose semantic information constraints. Accordingly, the paradigm outlined in Eq.~\ref{eq:problem_formulation} can be elaborated as follows:
% \begin{equation}
%     g_{s}\left ( \boldsymbol{u}; \boldsymbol{x}_{t} \right ) \Rightarrow \argmin_{u} \mathcal{D}\left ( e\left ( \boldsymbol{u}  \right ), e\left ( \boldsymbol{x}_{t}  \right )  \right ), \label{eq:semantic_constrain}
% \end{equation}
% where the \(\mathcal{D}\left( \cdot \right)\) represents the distance function measuring discrepancies between two edge maps, and \(e\left( \cdot \right)\) denotes the extraction of the edge map from a given modality. 

% For edge detection in frames \(\boldsymbol{x} \in \mathbb{R}^{hw}\), conventional edge extraction operators, such as the Canny detector, can be utilized. % to identify edges within frames. 
% However, the edge extraction from the motion representation \(\boldsymbol{u} \in \mathbb{R}^{hw \times d}\), which signifies offsets, presents a unique challenge. 
% Unlike RGB or depth images, \(\boldsymbol{u}\) cannot be straightforwardly processed using gradient-based methods due to its distinct nature representing offset. In this study, we categorize the edges within \(\boldsymbol{u}\) into two parts: intensity edges, where a significant change in offset magnitude occurs, and angular edges, marked by a notable shift in offset direction. These edge types can be articulated through the following representation:
% \begin{equation}
% \begin{aligned}
%     e\left ( \boldsymbol{u}  \right ) &= \left \{ \left ( i, j, \dots, k \right ) | \left | \nabla \left \| \boldsymbol{u} \right \|  \right |_{\left ( i,j,\dots, k \right ) } \ge \vartheta_{i} \right \} \\
%     &\cap \left \{ \left ( i, j, \dots, k \right ) | \left [ \frac{\vec{\boldsymbol{u}}_{\left ( i, j, \dots, k \right ) } \cdot \vec{\boldsymbol{u}}_{\left ( i+\delta , j+\delta, \dots, k+\delta \right ) }}{\left | \vec{\boldsymbol{u}}_{\left ( i, j, \dots, k \right ) } \right | \left | \vec{\boldsymbol{u}}_{\left ( i+\delta , j+\delta, \dots, k+\delta \right ) } \right | }    \right ] \le \vartheta_{a} \right \},
% \end{aligned}
% \end{equation}
% % where this formulation introduces an edge-extraction approach for multi-dimensional offsets. Here,
% where \(\vartheta_{i}\) and \(\vartheta_{a}\) are the thresholds for identifying intensity and angular edges, respectively, while \(\delta\) signifies a minimal coordinate shift. 
% As \(\boldsymbol{u}\) forms a dense vector field, variations within this field are expected to be continuous. Significant alterations in the magnitude of motion between adjacent points (\(\ge \vartheta_{i}\)) indicate changes in motion speed, whereas noticeable deviations in vector angles (\(\cos \le \vartheta_{a}\)) means directional changes. These insights help us to pinpoint and articulate motion edges differentiable, as illustrated by red lines in Fig.~\ref{fig:semantic}.

% Utilizing the edge points set derived from the \(\boldsymbol{u}\), we further elaborate on the distance metric \(\mathcal{D}\left( \cdot \right)\) as delineated in Eq.~\ref{eq:semantic_constrain}:
% \begin{equation}
%     \mathcal{D}\left ( e\left ( \boldsymbol{u}  \right ), e\left ( \boldsymbol{x}_{t}  \right )  \right ) = \sum_{p \in e\left ( \boldsymbol{u}  \right )} \min_{q \in e\left ( \boldsymbol{x}_{t}  \right )} \left \| p - q \right \|.
% \end{equation}
% For each point \(p\) in \(e\left ( \boldsymbol{u}  \right )\), we gain the nearest corresponding edge point \(q\) within \(e\left ( \boldsymbol{x}_{t} \right )\) and calculate their distance. These distances are denotes as white lines in Fig.~\ref{fig:semantic}.
% The accumulated distances quantifies the overall disparity between two edges.

% To make the computation of distance differentiable, we adopt the concept of differentiation to transition from a discrete to a continuous representation. This transformation involves segmenting the two sets of edge points into multiple regions within their spatial domain. Taking a 2D plane as an example, assume that within a certain region, the curves formed by the two sets of points are denoted as \(\mathcal{C}_{1}\) and \(\mathcal{C}_{2}\), with their abscissa distributed within the interval \(\left [ a, b \right ] \). As shown in Fig.~\ref{fig:semantic}, the distance between these two curves can then be approximated by the following formulation:
% \begin{equation}
% \begin{aligned}
%     \mathcal{D}(\mathcal{C}_{1}, \mathcal{C}_{2}; [a, b]) = &\sum_{n=1}^{\infty} \sum_{i=0}^{2^n-1} \Phi \left(\mathcal{C}_{1}, \mathcal{C}_{2}; \left[a + \frac{i(b-a)}{2^n}, a + \frac{(i+1)(b-a)}{2^n}\right]\right), \\
%     & +\Phi(\mathcal{C}_{1}, \mathcal{C}_{2}; [a, b]), \label{eq:curve_distance}
% \end{aligned}
% \end{equation}
% where the \(\Phi()\) %signifies the function for calculating 
% calculates the distance between the centroids of these curves, % This computation is 
% detailed as:
% \begin{equation}
%     \Phi(\mathcal{C}_{1}, \mathcal{C}_{2}; [m, n]) = \left\Vert \left(\bar{x}_{\mathcal{C}_{1}}, \bar{y}_{\mathcal{C}_{1}}\right) - \left(\bar{x}_{\mathcal{C}_{2}}, \bar{y}_{\mathcal{C}_{2}}\right) \right\Vert_2,
% \end{equation}
% and assuming the curves can be described by a function \(h\), the centroids are determined by:
% \begin{equation}
%     \bar{x}_{h} = \frac{\int_{m}^{n} x \cdot h(x) \, dx}{\int_{m}^{n} h(x) \, dx},
%     \bar{y}_{h} = \frac{1}{2} \cdot \frac{\int_{m}^{n} h(x)^2 \, dx}{\int_{m}^{n} h(x) \, dx}.
% \end{equation}
% Through this approximation, we achieve a continuous method for calculating the distance between two curves, serving as an implementation of semantic constraint.

% \paragraph{Kinematic Constraint with Skeletal Motion:} In human-centric motion representation, alongside precise semantic information, the accuracy of motion information is equally crucial. This accuracy directly impacts the model's ability to precisely identify specific patterns, especially during complex or subtle motion changes, which is particularly important in tasks of action analysis, biometric studies, medical diagnostics, etc. 
% To capture motion information, the movement of the human skeleton offers a significant representation. Therefore, assuming \(\boldsymbol{k}_{t} \in \mathbb{R}^{n \times d}\) denotes the \(n\)-points skeletal position in frame \(\boldsymbol{x}_{t}\) in either \(2\) or more dimension space, the 
% \(g_k\) in Eq.~\ref{eq:problem_formulation} can be further detailed as:
% \begin{equation}
%     g_{k}\left ( \boldsymbol{u}; \boldsymbol{x}_{t} \rightarrow \boldsymbol{x}_{t+1}  \right ) \Rightarrow \arg\min_{\boldsymbol{u}}\mathcal{F}\left ( \boldsymbol{u}, \boldsymbol{k}_{t} \rightarrow \boldsymbol{k}_{t+1} \right ), \label{eq:kinematic_constrain}
% \end{equation}
% where \(\mathcal{F}\left( \cdot \right)\) denotes the degree of misalignment between \(\boldsymbol{u}\) and the skeletal displacements across consecutive frames.
% % displacements or removal?

% Unlike prior works that construct stick-figure removal from skeletal offsets to serve as the ground truth, our method aims to preserve semantic information and address potential faults in pose estimation. To this end, we employ a dynamic approach for correlating keypoints, thereby calculating such discrepancies. Specifically, for any point \(p \in \boldsymbol{u}\), we identify its corresponding skeletal keypoint \(\hat{q}\) via:
% \begin{equation}
%     \hat{q} = \argmin_{q \in \boldsymbol{k}_{t}\cdot{s}} \left( \left\| p, q \right\| * -{c}_{q}\right), ~\ \mathit{s.t.} ~\ p \in \boldsymbol{u}\cdot{s}. 
% \end{equation}
% Here \(c_{q}\) represents the visibility and confidence. 
% The \(\cdot{s}\) indicates that this matching is confined to the area occupied by subject \(s\), thus preventing incorrect voxel matches in \(\boldsymbol{u}\) in multi-person scenarios. % with multiple individuals.

% By exploiting the alignment between the \(\boldsymbol{u} \in \mathbb{R}^{hw \times d}\) and skeletal offsets \(\vec{\boldsymbol{k}} = \boldsymbol{k}_{t} \rightarrow \boldsymbol{k}_{t+1} \in \mathbb{R}^{n \times d}\) at the time \(t\), in conjunction with the biomechanical priors of human anatomy that the trajectory of muscular motion cannot be orthogonal to the skeletal movement trajectory, we are poised to further delineate the function \(\mathcal{F}\left(\cdot \right)\) as follows:
% \begin{equation}
%     \mathcal{F}\left ( \boldsymbol{u}, \vec{\boldsymbol{k}} \right ) = \frac{1}{\boldsymbol{u}} \sum_{p \in \boldsymbol{u}} \mathbb{I}\left [ \frac{\boldsymbol{u}_{p}\cdot \vec{\boldsymbol{k}}_{\hat{q}}}{\left | \boldsymbol{u}_{p} \right | \cdot \left | \vec{\boldsymbol{k}}_{\hat{q}} \right | } \le \vartheta_{k} \right ] 
% + \operatorname{ReLU}\left[\left(\boldsymbol{u}_{p}-\vartheta_{i}^{l} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right) \cdot\left(\boldsymbol{u}_{p}-\vartheta_{i}^{h} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right)\right]. \label{eq:kinematic}
% \end{equation}
% As depicted in Fig.~\ref{fig:kinematic}, the muscular motion \(\boldsymbol{u}_{p}\) (pink vector) is constrained by skeletal motion \(\vec{\boldsymbol{k}}_{\hat{q}}\) (cyan vector). The sector shaded with blue lines represents our angular constraint, where \(\vartheta_{k}\) delineates the allowable angle between \(\boldsymbol{u}_{p}\) and \(\vec{\boldsymbol{k}}_{\hat{q}}\). The annular region depicted with purple lines denotes the intensity constraint, with \(\vartheta_{i}^{l}\) and \(\vartheta_{i}^{h}\) defining the lower and upper bounds of motion intensity for \(\boldsymbol{u}_{p}\) relative to \(\vec{\boldsymbol{k}}_{\hat{q}}\). As such, through the formulation expressed in Eq.~\ref{eq:kinematic}, we ensure that \(\boldsymbol{u}_{p}\) falls within the green zone, satisfying both intensity and angular constraints.
% % wherein \(\vartheta_{k}\) specifies the threshold angle that delineates the directional congruence between muscular and skeletal motions. The parameters \(\vartheta_{i}^{l}\) and \(\vartheta_{i}^{h}\) define the lower and upper boundaries of motion intensity relative to skeletal displacement, respectively. The function \(\mathbb{I}\) denotes the indicator function. This formulation integrates a dynamic constraint on skeletal motion, thereby enabling the generation of a motion representation enriched with semantic and kinematic information.

\subsection{Joint Constraint Learning Framework {\footnotesize \mfinish{Oct.14}}} \label{sec:joint_constraint}

In our proposed self-supervised learning \com{We did not mention that in Eq. 2.} framework introduced in \cref{eq:world_constraint}, the two regularization terms, namely the Skeleton-Muscle Constraint for determining the general range of motion and the Edge-Chamfer Constraint for refining motion details and incorporating human shape information, both involve numerous discrete operation. In this part, we will discuss these constraints in detail, elaborating on how we transform these discrete operations into differentiable matrix computations.

\vspace{2pt}
\noindent\textbf{\textit{Skeleton-Muscle Constraint:}} In action analysis tasks, the accuracy of motion information is crucial, as it directly affects the model's ability to recognize specific patterns, especially in tasks involving complex or subtle motion changes, such as action analysis. To capture kinematic information effectively, skeletal offsets provide valuable insights.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/skeletal_constraint.pdf}
  \caption{Skeletal Constraint}
  \label{fig:skeleton_constraint}
\end{figure}

Unlike PoseFlow~\cite{zhang2018poseflow}, which directly constructs pseudo ground truth based on skeletal offsets, we aim to reduce the influence of errors from skeleton estimation on flow estimation while preserving as much human shape information as possible. To achieve this, we establish a dynamic relationship between the skeleton and muscle points, thereby creating a kinematic fidelity constraint. We begin by using 2D pose estimation algorithms, such as ED-Pose~\cite{yang2022explicit}, to extract joint points \( \mathbb{R}^{17 \times 3} \) from frame \( \boldsymbol{x}_t \), and utilize interpolation to construct a skeleton map with confidence \( \boldsymbol{k}_{t} \in \mathbb{R}^{N_{k} \times 3} \). Each bone segment is uniformly sampled, typically consisting of more than 200 points (\( N_{k} \geq 200 \)). Then, for any muscle point \( p \in \boldsymbol{u} \), we identify the closest corresponding keypoint \( \hat{q} \) in the skeleton map by minimizing a weighted distance. This process is formulated as:
\begin{equation}
    \hat{q} = \arg\min_{q \in \boldsymbol{k}_{t} \cdot s} \left( \left\| p - q \right\| * -{v}_{q}\right), ~\ \mathit{s.t.} ~ p \in \boldsymbol{u} \cdot s,
    \label{eq:skeleton_match}
\end{equation}
where \( v_{q} \) represents the visibility and confidence of the point \( q \). The \( \cdot s \) restricts matching to the region occupied by subject \( s \), avoiding incorrect voxel matches in \( \boldsymbol{u} \) in multi-person scenarios. Typically, \( \hat{q} \) is the perpendicular projection from \( p \) to the nearest skeletal segment.

Through this skeleton-muscle matching, we are able to construct our dynamic constraint. Based on human biological priors, we infer that, for any point \( p \) on a muscle, its movement direction will not be orthogonal to that of its corresponding skeletal points \( \hat{q} \), nor will it exhibit a significantly different motion intensity. Therefore, we construct our skeleton-muscle constraint that includes both angular and intensity constraints to create a kinematic fidelity term for each \( \left \langle p - \hat{q} \right \rangle  \) pair. Based on the cosine theorem, we can calculate the angle formed by the vectors \( \boldsymbol{u}_{p} \) and \( \vec{\boldsymbol{k}}_{\hat{q}} \), and constrain it to be less than a given threshold \( \vartheta_{a} \) to construct the angular constraint as:
\begin{equation}
    \mathcal{F}_{A}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) = \mathbb{I}\left ( \frac{\boldsymbol{u}_{p}\cdot \vec{\boldsymbol{k}}_{\hat{q}}}{\left | \boldsymbol{u}_{p} \right | \cdot \left | \vec{\boldsymbol{k}}_{\hat{q}} \right | } \geq \vartheta_{a} \right ),
    \label{eq:angular_constraint}
\end{equation}
where \( \vec{\boldsymbol{k}} \in \mathbb{R}^{n_{k} \times 3} \) represents the offset between two skeletal maps, which can be calculated as \( \boldsymbol{k}_{t} - \boldsymbol{k}_{t+1} \). The term \( \mathbb{I} \left( \cdot \right) \) is the indicator function, used to count abnormal points. Besides, we require the motion intensity at a muscle point \( p \) to fall within a dynamic range based on the intensity of the corresponding skeletal point \( \hat{q} \), which can be formulated by:
\begin{equation}
    \mathcal{F}_{I}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) = \operatorname{ReLU}\left[\left(\boldsymbol{u}_{p}-\vartheta_{i}^{l} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right) \cdot\left(\boldsymbol{u}_{p}-\vartheta_{i}^{h} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right)\right],
    \label{eq:intensity_constraint}
\end{equation}
which means that when the ratio between the two offsets falls outside the range \( \left[ \vartheta_{i}^{l}, \vartheta_{i}^{h} \right] \), a penalty value will be applied as the constraint. Hence, the \( \mathcal{F} \) in \cref{eq:world_constraint} can be further detailed as:
\begin{equation} % \left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right )
    \mathcal{F} = \frac{1}{h \cdot w} \sum_{p \in \boldsymbol{u}} \left[ \mathcal{F}_{A}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) + \beta \cdot \mathcal{F}_{I}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) \right ],
    \label{eq:skeleton_muscle_constraint}
\end{equation}
where \( \beta \) is used for trade-off.

\vspace{2pt}
\noindent\textbf{\textit{Edge-Chamfer Constraint:}} Similarity\com{Do you mean similarly?}, human shape information, particularly the boundaries, plays a crucial role in action analysis tasks~\cite{tseng2023edge, chai2022lagrange, pham2022video}. Human shape information can significantly enhance the analysis models' ability to locate different body patterns, thereby improving recognition accuracy. For instance, in 3D reconstruction tasks~\cite{ye2023nef, schmied2023r3d3}, shape information aids in accurately estimating the body structure. Further, in scenarios with complex backgrounds or multiple subjects, boundaries help distinguish between individuals~\cite{he2020bdcn}. Given these considerations, we employ human boundaries to constrain the edges of the flow map \( \boldsymbol{u} \).

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/edge_constraint.pdf}
  \caption{Edge-Chamfer Constraint}
  \label{fig:edge_constraint}
\end{figure}

Edge detection \com{Why all of sudden we start to talk about edge detection?} on visible images has numerous well-established algorithms, such as gradient calculation or the Canny operator. In contrast, defining and extracting edges from a flow map is more challenging. We represent the edges of flow map  \( \boldsymbol{u} \) as a set of discontinuity points \( \boldsymbol{s} \), which can be categorized into intensity and angular discontinuities. Intensity discontinuities occur when the offset between point \(p\) and its neighboring point \(j\) has a substantial difference in magnitude (\( \geq \vartheta_{i} \)), such as between a moving foreground and a static background, which can be represented as:
\begin{equation}
    \boldsymbol{s}_{I} = \left \{ p \in \boldsymbol{u} \mid \left | \boldsymbol{u}_{p} - \boldsymbol{u}_{j} \right |   \ge \vartheta_{i} \right \}.
    \label{eq:intensity_edge}
\end{equation}
On the other hand, angular discontinuities refer to scenarios where the offset between \(p\) and \(j\) exhibits a significant difference in angle (\( \geq \vartheta_{a} \)), typically occurring between different body patterns, which can be represented as:
\begin{equation}
    \boldsymbol{s}_{A} = \left \{ p \in \boldsymbol{u} \mid \frac{\boldsymbol{u}_{p}\cdot \boldsymbol{u}_{j}}{\left | \boldsymbol{u}_{p} \right | \cdot \left | \boldsymbol{u}_{j} \right | } \geq \vartheta_{a} \right \}.
    \label{eq:angular_edge}
\end{equation}
Therefore, for any flow map \( \boldsymbol{u} \), its edge map \( \boldsymbol{s} \) can be formulated by \( \boldsymbol{s}_{I} \cup \boldsymbol{s}_{A} \).

Chamfer distance is often used to measure the distance between two sets of curves. For instance, when measuring the distance between flow edge map \(\boldsymbol{s}\) and human boundaries \(\boldsymbol{e}\), it can be defined as the sum of the nearest distances from any point \(p \in \boldsymbol{s}\) to \(\boldsymbol{e}\). This process can be represented by:
\begin{equation}
    \begin{gathered}
        \mathcal{C}\left( \boldsymbol{s}, \boldsymbol{e} \right) = \sum_{p \in \boldsymbol{s}} \mathcal{D}\left( p, \hat{q} \right), \,
        \text{s.t.} \, \hat{q} = \arg\min_{q \in \boldsymbol{e}} \mathcal{D}\left( p, q \right),
        \label{eq:chamfer_distance}
    \end{gathered}
\end{equation}
where \( \mathcal{D}\left( \cdot \right) \) denotes the Euclidean distance between two points. However, a significant issue is that the operation of finding matching points is inherently discrete. Searching for matching pairs \( \langle p, q \rangle \) between the two dense maps \( \boldsymbol{s} \) and \( \boldsymbol{e} \) requires substantial computation. 

Therefore, we design a method to replace these discrete calculations with matrix operations, namely patch-centroid distance. Based on the concept of calculus, we use kernels with different receptive field sizes to divide both \( \boldsymbol{s} \) and \( \boldsymbol{e} \) into multiple patches across various scales. For any given patch \(\mathcal{P}\), the Chamfer distance between the two curves within that patch (\(\mathcal{P}_{\boldsymbol{s}}\) and \(\mathcal{P}_{\boldsymbol{e}}\)) can be approximated by calculating the distance between the centroids \( \boldsymbol{c} \) of each curve within the patch's boundaries when the point set distribution is smooth. This approximation can be derived through:
\begin{equation}
    \begin{aligned}
        \mathcal{C}\left( \mathcal{P}_{\boldsymbol{s}}, \mathcal{P}_{\boldsymbol{e}} \right) &= \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle }\mathcal{D}\left ( p, \hat{q} \right ) 
        \\ &\approx \mathcal{D}\left ( \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle } p,  \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle } \hat{q} \right ) 
        \\ &\approx \mathcal{D}\left ( \boldsymbol{c}_{\mathcal{P}_{\boldsymbol{s}}}, \boldsymbol{c}_{\mathcal{P}_{\boldsymbol{e}}} \right ) 
        \label{eq:patch_centroid_distance}
    \end{aligned}
\end{equation}
where \(N_p\) denotes the total number of point pairs. Hence, the \( \mathcal{G} \) in \cref{eq:world_constraint} can be further detailed as:
\begin{equation} % \left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right )
    \mathcal{G} = \frac{1}{N_{ms}}\sum_{ms}\left [ \frac{1}{N_{\mathcal{P}}} \sum_{\mathcal{P}\propto ms} \mathcal{C}\left( \mathcal{P}_{\boldsymbol{s}}, \mathcal{P}_{\boldsymbol{e}} \right)  \right ],
    \label{eq:edge_chamfer_constraint}
\end{equation}
where the \(N_{ms}\) and \(N_{\mathcal{P}}\) denotes the depth of multi-scale mechanism and the amount of patches under corresponding scale (\(ms\)), respectively.


\subsection{Dual Coordinate Flow Estimation {\footnotesize \mfinish{Oct.14}}} \label{sec:dual_coord}

% \begin{figure}[t]
%   \centering
%   \includegraphics[trim=0 0 0 0,clip,width=\textwidth]{assets/network.png}
%   \caption{Overview of the Proposed HuMoR Estimation Pipeline. {\small This figure illustrates the pipeline of our method, which centers around the dual-coordinate flow estimation network, \(\mathcal{N}_{flow}\), framed by the blue dotted line. The network is specifically designed for estimation human motion, which operates under the guidance of our semantic \(g_s\) and kinematic \(g_k\) joint constraint learning, represented by the brown and green regions, respectively.}} 
%   \label{fig:network}
%   \vspace{-12pt}
% \end{figure}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{asset/network_architecture.pdf}
  \caption{}
  \label{fig:whole_pipeline}
\end{figure*}

By expanding \cref{eq:world_constraint} with the equations derived from \cref{eq:skeleton_muscle_constraint} and \cref{eq:edge_chamfer_constraint}, we can utilize a self-supervised approach to learn the offset of muscle points in the world coordinate system from real-world scenarios, which corresponds to the concept of World Motion (\( \boldsymbol{u_w} \)) introduced in \cref{sec:problem_formulation}. In some action analysis tasks, in fact, from a human point of view, they rely more on analyzing the internal motion than on the interaction between the human body and the scene, such as analyzing the gait of a pedestrian or the diving process of an athlete. Therefore, we introduce the concept of Local Flow (\( \boldsymbol{u_l} \)) to better capture these potential motion states. Together with World Motion, our Dual Coord. Flow allow the analysis model to think in the same way as the human kinematic analysis process, providing a novel possibility for the establishment of the world model.

In \cref{eq:dual_coord_flow}, we discussed the relationship between \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \). To obtain both of them, which together from our Dual Coord. Flow,
we avoid using two flow estimation network \(\Phi\) independently to estimate \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \). Instead, we leverage the principle of vector decomposition. By using a single flow estimation network \(\Phi\) to estimate \( \boldsymbol{u_w} \), and a shallow network \(\Psi\) to estimate \( \boldsymbol{u_s} \), we indirectly solve for \( \boldsymbol{u_l} \). This approach significantly reduces the computational load during both training and inference, this process can be formulated by:
\begin{equation}
    \begin{aligned}
        \Phi \left( \omega_{1}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) &\Rightarrow \boldsymbol{u_w},
        \\ \Psi \left( \omega_{2}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}, \boldsymbol{u_w} \right) &\Rightarrow \boldsymbol{u_s},
        \\ \boldsymbol{u_w} - \boldsymbol{u_s} &= \boldsymbol{u_l}.
    \end{aligned}
\end{equation}

Since we use different reference systems, \cref{eq:world_constraint}, which constrains \( \boldsymbol{u_w} \), requires transformations to be applicable for constraining \( \boldsymbol{u_l} \). Specifically, this transformation affects \( \vec{\boldsymbol{k}} \) in \cref{eq:skeleton_muscle_constraint}. In \cref{sec:joint_constraint}, \( \vec{\boldsymbol{k}} \) represents the offsets between two skeletal maps (\( \boldsymbol{k}_t \) and \(\boldsymbol{k}_{t+1} \)), which is defined with respect to the ground. Therefore, we need to convert this displacement to be relative to the subject itself, which can be achieved by aligning \( \boldsymbol{k}_t \) and \( \boldsymbol{k}_{t+1} \). We propose two alignment methods to achieve this. The first is homography-based matching, which calculates a transformation matrix to minimize the overall offsets between \( \boldsymbol{k}_t \) and \( \boldsymbol{k}_{t+1} \) through an analytical solution. By applying this transformation to \( \boldsymbol{k}_{t+1} \), alignment with \( \boldsymbol{k}_t \) can be accomplished, which proves effective in most scenarios. However, for some specific tasks such as analyzing diving sequences, where rotational motion is dominant, the homography-based matching may lead to skeletal distortions. For these cases, we design a head-aligned based alignment approach. In this method, \( \boldsymbol{k}_{t+1} \) is rotated to align its head keypoints as closely as possible with those of \( \boldsymbol{k}_t \). After applying either of these two alignment methods, we obtain adjusted skeletal map \( \boldsymbol{k}_{t+1}' \), from which we derive the subject-relative offsets \( \vec{\boldsymbol{k}'} \). Based on this, we transfer \( \mathcal{F} \) to \( \mathcal{F}'\). Thus, similar to \cref{eq:world_constraint}, the constraint for \( \boldsymbol{u_l} \) can be represented as:
\begin{equation}
    \boldsymbol{u_l} =  \arg\min_{\boldsymbol{u}}\left [ \mathcal{F}'\left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + \alpha \cdot \mathcal{G}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right ) \right ]. \label{eq:local_constraint}
\end{equation}
Based on \cref{eq:world_constraint} and \cref{eq:local_constraint}, we can determine the optimal values for \( \omega_{1} \) in \( \Phi \) and \( \omega_{2} \) in \( \Psi \) by applying the chain rule of differentiation.



%
% NeuIPS version
%
% By expanding the constraints in Eq.~\ref{eq:problem_formulation}, we can learn a precision motion about human from real-world scenarios.
% As highlighted in Eq.~\ref{eq:multi_coordinate}, some action analysis rely more on the intrinsic motions of humans rather than interactions within the scene, such as in gait recognition and action recognition tasks. Therefore, we introduce the concept of local reference frames to capture these internal dynamics.
% % Inspired by kinematic analysis in physics, we recognize that certain downstream tasks, such as gait recognition, require a more detailed local-based analysis of human motion. 
% % Therefore, %to provide a stable and accurate perception of these tasks,
% % we introduce the concept of local reference frames. 
% To estimate the offset \(\boldsymbol{m}\) of the local coordinate system's origin relative to the global coordinate one in Eq.~\ref{eq:problem_formulation}, we utilize the skeletal position information in adjacent frames. Thus, Eq.~\ref{eq:multi_coordinate} can be detailed as:
% \begin{equation}
%     \boldsymbol{u^l} = \boldsymbol{u^w} - \left [ \boldsymbol{k}_{t+1}-\argmin_{\mathcal{T}\left ( {\boldsymbol{k}_{t+1}} \right ) } \left ( \sum_{i \in \boldsymbol{k_{*}}} \left \| \boldsymbol{k}_{t}^{i} - \mathcal{T}\left ( \boldsymbol{k}_{t+1} \right ) ^{i}\right \|   \right )  \right ], \label{eq:coord_transfer}
% \end{equation}
% where \(\mathcal{T}\left(\cdot \right)\) represents the constrained transformation applied to the skeleton, such as a scale-translate transformation (for motion within the same plane) and a projective transformation (for 3D motion). Therefore, by computing human motion under the world coordinate system, denoted by HuMoR {\scriptsize W.} (\(\boldsymbol{u^{w}}\)), and factoring in the local coordinate shift \(\boldsymbol{m}\), we can accurately determine the human motion relative to itself, represented as HuMoR {\scriptsize L.} (\(\boldsymbol{u^{l}}\)).
% % Therefore, by computing human motion under the world coordinate system, HuMoR {\scriptsize W.} \(\boldsymbol{u^{w}}\), and local coordinate shift \(\boldsymbol{m}\), we can discern human motion relative to itself, HuMoR {\scriptsize L.} \(\boldsymbol{u^{l}}\).

% Leveraging the robust fitting capability of neural networks, the function \(f\left ( \boldsymbol{u}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right )\) in Eq.~\ref{eq:problem_formulation} can be implemented by constructing \(\mathcal{N}_{flow} \left \langle \mathcal{N}_{b}, \mathcal{N}_{t} \right \rangle \) (as shown in Fig.~\ref{fig:network}). For the \(\boldsymbol{u^w} = \mathcal{N}_{b}\left( \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right)\), based on Eq.~\ref{eq:semantic_constrain} and Eq.~\ref{eq:kinematic_constrain}, the two constraints, \(g_s\) and  \(g_k\), can be expressed as the loss function:
% \begin{equation}
%     \mathcal{L}_{\boldsymbol{u^{w}}} = \mathcal{D}\left [ e\left ( \boldsymbol{u^{w}}  \right ), \operatorname{Canny}\left ( \mathcal{N}_{s}\left ( \boldsymbol{x}_{t}  \right )  \right )\right ] + \alpha \cdot \mathcal{F}\left [ \boldsymbol{u}, \mathcal{N}_{p}\left ( \boldsymbol{x}_{t}  \right ) \rightarrow \mathcal{N}_{p}\left ( \boldsymbol{x}_{t+1}  \right ) \right ],
% \end{equation}
% where \(\mathcal{N}_{s}\) and \(\mathcal{N}_{p}\) denote the semantic segmentation and pose estimation networks, respectively, and \(\alpha\) is a trade-off hyper-parameter.

% Moreover, during the forward derivation process, by utilizing high-dimensional features \(\gamma\) inherent in the \(\mathcal{N}_{b}\), we can estimate the shift of the local coordinate origin directly from adjacent frames end-to-end, thus avoiding the use of additional networks (e.g., human detection or pose estimation) during inference. For the \(\boldsymbol{m} = \mathcal{N}_{t}\left( \boldsymbol{u_w}, \gamma \right)\), based on Eq.~\ref{eq:coord_transfer}, this part of the loss formula can be:
% \begin{equation}
%     \mathcal{L}_{\boldsymbol{m}} = \left \| \boldsymbol{m}, \left [ \mathcal{N}_{p}\left ( \boldsymbol{x}_{t+1} \right ) - \mathcal{T}\left ( \mathcal{N}_{p}\left ( \boldsymbol{x}_{t+1} \right ) \right )  \right ] \right \|.
% \end{equation}

% Finally, we can obtain highly representative representations of human-related motion across multiple analysis viewpoints by developing this human motion estimation network based on s-k joint constraint within a dual coordinate system. These representations can enhance the accuracy of subsequent motion analysis algorithms, whether their analysis relies on global or local movements.

==> section/03_method_v2.tex <==
\section{Methodology \mfinish{Oct.31} {\small \TODO{Updating}}}

\subsection{Problem Formulation {\footnotesize \mfinish{Oct.31}}} \label{sec:problem_formulation}

\com{One sentence about the overall goal is missing here. We need to state that the goal is to learn human-centric motion representation by extracting human motion from noisy optical flow using human pose as a prior.}

\com{I STRONGLY suggest we don't talk about local flow in this paragraph because it is way too much. Let's first focus on explaining the two constraints first. Try this line of logic in this subsection: 1) What is our solution. We propose a joint constraint framework to learn human-centric motion representation. 2) Why this motion representation is human centric. This is because this motion representation is learned from two constraints. 3) What do the two constraints do. One for skeleton and the other is for body. 4) The world flow is not good enough and why. We then use these two constraints to learn both world flow and local flow. 5) What is the benefit of using two flows. 
6) How the world flow and local flow are combined to build the motion representation. You may use equations to further explain some details.}
To learn human-centric motion representation from real-world scenarios, which contains precise human motion and detailed shape information, \methodName{} introduce a Joint Constraint framework to learning World-Local Flows (W-L Flows) from adjacent frames. Given any pair of consecutive frames \( \left( \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) \), \methodName{} estimates the motion relevant to the external environment, termed World Flow \(\boldsymbol{u_w}\) and the motion relative to subject's own body, termed Local Flow \(\boldsymbol{u_l}\). Specifically, the estimation process is divided into two parts. As the most prominent motion information, \(\boldsymbol{u_w}\) can be directly inferred from adjacent frames. Meanwhile, \(\boldsymbol{u_l}\), serving as underlying information, requires additional calculation for indirect derivation.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/whole_pipeline.pdf}
  \caption{Joint Constraint}
  \label{fig:joint_constraint}
\end{figure}

As illustrated in \cref{fig:joint_constraint}, our target is to find the flow map with the most accurate motion and shape information \(\boldsymbol{u_w}\) (white ball) from all possible flow maps \(\boldsymbol{u} = \Phi \left( \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}; \omega_{1} \right)\) (cube). The \( \Phi \) and \( \omega_{1} \) represent a flow estimation network and its corresponding parameters, respectively. 

For this purpose, we introduce two fidelity terms, termed skeletal constraint \(\mathcal{F}\) and boundary constraint \(\mathcal{G}\). The skeletal constraint ensures the movement of each body point adheres to realistic physiological constraints, \eg the coordination between body and skeletal movements. Specifically, \(\mathcal{F}\) measures the difference between the estimated \(\boldsymbol{u}\) and the pose offset between \(\boldsymbol{x}_{t}\) and \(\boldsymbol{x}_{t+1}\). Additionally, the boundary constraint preserves human shape information. In particular, this magnifies the difference between the boundary of humans in \(\boldsymbol{u}\) and \(\boldsymbol{x}_{t}\).

The optimal solution sets of both, where the regularization loss is zero, manifest as an irregular continuous surface in high-dimensional space, abstract as a 3D saddle surface (blue for skeletal, pink for boundary) in \cref{fig:joint_constraint}. Hence, our target \(\boldsymbol{u_w}\) can be represented as the point closest to both saddle surfaces. Therefore, our Joint Constraint framework can be represented as:
\begin{equation}
    \boldsymbol{u_w} =  \arg\min_{\boldsymbol{u}}\left [ \mathcal{F}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + \alpha \cdot \mathcal{G}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right ) \right ], \label{eq:world_constraint}
\end{equation}
where \( \alpha \) is a weight used for a trade-off.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/wl_flows.pdf}
  \caption{World-Local Flows\com{more text is needed to explain this figure.}}
  \label{fig:wl_flows}
\end{figure}

At this point, we have obtained the prominent motion, \ie world flow \(\boldsymbol{u_w}\), applicable to most action analysis tasks. However, for tasks requiring deeper motion information, \eg gait recognition, we need to provide further insights for human-centric motion. We draw inspiration from physical kinematics and introduce a concept similar to Galilean Transformation~\cite{}. Different from the world flow \(\boldsymbol{u_w}\) which represents the offset of each point relative to the ground, we introduce the local flow \(\boldsymbol{u_l}\). This represents the relative offset with respect to the moving subject itself. Directly calculating \(\boldsymbol{u_l}\) from adjacent frames is challenging, instead, we utilize vector decomposition to estimate it indirectly.

As the actual offset information, world flow \(\boldsymbol{u_w}\) can be viewed as the resultant of the subject's overall motion \(\boldsymbol{u_s}\) and \(\boldsymbol{u_l}\), demonstrated in \cref{fig:wl_flows}. Therefore, given \(\boldsymbol{u_w}\), we can indirectly obtain \(\boldsymbol{u_l}\) by estimating \(\boldsymbol{u_s}\), denoted as:
\begin{equation}
    \begin{gathered}
        \boldsymbol{u_l} = \boldsymbol{u_w} - \boldsymbol{u_s}, \\
        \boldsymbol{u_s} = \Psi \left(\boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}, \boldsymbol{u_w}; \omega_{2} \right),
    \end{gathered}
    \label{eq:wl_flow}
\end{equation}
where the \( \Psi \) denotes the network used to estimate \( \boldsymbol{u_s} \) based on frames and \( \boldsymbol{u_w} \), \( \omega_{2} \) represents parameters in \( \Psi \).

\subsection{Joint Constraint Learning Framework {\footnotesize \mfinish{Oct.14}}} \label{sec:joint_constraint}

In our proposed self-supervised learning \com{We did not mention that in Eq. 2.} framework introduced in \cref{eq:world_constraint}, the two regularization terms, namely the Skeleton-Muscle Constraint for determining the general range of motion and the Edge-Chamfer Constraint for refining motion details and incorporating human shape information, both involve numerous discrete operation \com{This is another super long sentence}. In this part \com{subsection}, we will discuss these constraints in detail, elaborating on how we transform these discrete operations into differentiable matrix computations.

\vspace{2pt}
\noindent\textbf{\textit{Skeleton-Muscle Constraint:}} In action analysis tasks, the accuracy of motion information is crucial, as it directly affects the model's ability to recognize specific patterns, especially in tasks involving complex or subtle motion changes, such as action analysis. To capture kinematic information effectively, skeletal offsets provide valuable insights.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/skeletal_constraint.pdf}
  \caption{Skeletal Constraint}
  \label{fig:skeleton_constraint}
\end{figure}

Unlike PoseFlow~\cite{zhang2018poseflow}, which directly constructs pseudo ground truth based on skeletal offsets, we aim to reduce the influence of errors from skeleton estimation on flow estimation while preserving as much human shape information as possible. To achieve this, we establish a dynamic relationship between the skeleton and muscle points, thereby creating a kinematic fidelity constraint. We begin by using 2D pose estimation algorithms, such as ED-Pose~\cite{yang2022explicit}, to extract joint points \( \mathbb{R}^{17 \times 3} \) from frame \( \boldsymbol{x}_t \), and utilize interpolation to construct a skeleton map with confidence \( \boldsymbol{k}_{t} \in \mathbb{R}^{N_{k} \times 3} \). Each bone segment is uniformly sampled, typically consisting of more than 200 points (\( N_{k} \geq 200 \)). Then, for any muscle point \( p \in \boldsymbol{u} \), we identify the closest corresponding keypoint \( \hat{q} \) in the skeleton map by minimizing a weighted distance. This process is formulated as:
\begin{equation}
    \hat{q} = \arg\min_{q \in \boldsymbol{k}_{t} \cdot s} \left( \left\| p - q \right\| * -{v}_{q}\right), ~\ \mathit{s.t.} ~ p \in \boldsymbol{u} \cdot s,
    \label{eq:skeleton_match}
\end{equation}
where \( v_{q} \) represents the visibility and confidence of the point \( q \). The \( \cdot s \) restricts matching to the region occupied by subject \( s \), avoiding incorrect voxel matches in \( \boldsymbol{u} \) in multi-person scenarios. Typically, \( \hat{q} \) is the perpendicular projection from \( p \) to the nearest skeletal segment.

Through this skeleton-muscle matching, we are able to construct our dynamic constraint. Based on human biological priors, we infer that, for any point \( p \) on a muscle, its movement direction will not be orthogonal to that of its corresponding skeletal points \( \hat{q} \), nor will it exhibit a significantly different motion intensity. Therefore, we construct our skeleton-muscle constraint that includes both angular and intensity constraints to create a kinematic fidelity term for each \( \left \langle p - \hat{q} \right \rangle  \) pair. Based on the cosine theorem, we can calculate the angle formed by the vectors \( \boldsymbol{u}_{p} \) and \( \vec{\boldsymbol{k}}_{\hat{q}} \), and constrain it to be less than a given threshold \( \vartheta_{a} \) to construct the angular constraint as:
\begin{equation}
    \mathcal{F}_{A}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) = \mathbb{I}\left ( \frac{\boldsymbol{u}_{p}\cdot \vec{\boldsymbol{k}}_{\hat{q}}}{\left | \boldsymbol{u}_{p} \right | \cdot \left | \vec{\boldsymbol{k}}_{\hat{q}} \right | } \geq \vartheta_{a} \right ),
    \label{eq:angular_constraint}
\end{equation}
where \( \vec{\boldsymbol{k}} \in \mathbb{R}^{n_{k} \times 3} \) represents the offset between two skeletal maps, which can be calculated as \( \boldsymbol{k}_{t} - \boldsymbol{k}_{t+1} \). The term \( \mathbb{I} \left( \cdot \right) \) is the indicator function, used to count abnormal points. Besides, we require the motion intensity at a muscle point \( p \) to fall within a dynamic range based on the intensity of the corresponding skeletal point \( \hat{q} \), which can be formulated by:
\begin{equation}
    \mathcal{F}_{I}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) = \operatorname{ReLU}\left[\left(\boldsymbol{u}_{p}-\vartheta_{i}^{l} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right) \cdot\left(\boldsymbol{u}_{p}-\vartheta_{i}^{h} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right)\right],
    \label{eq:intensity_constraint}
\end{equation}
which means that when the ratio between the two offsets falls outside the range \( \left[ \vartheta_{i}^{l}, \vartheta_{i}^{h} \right] \), a penalty value will be applied as the constraint. Hence, the \( \mathcal{F} \) in \cref{eq:world_constraint} can be further detailed as:
\begin{equation} % \left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right )
    \mathcal{F} = \frac{1}{h \cdot w} \sum_{p \in \boldsymbol{u}} \left[ \mathcal{F}_{A}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) + \beta \cdot \mathcal{F}_{I}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) \right ],
    \label{eq:skeleton_muscle_constraint}
\end{equation}
where \( \beta \) is used for trade-off.

\vspace{2pt}
\noindent\textbf{\textit{Edge-Chamfer Constraint:}} Similarity\com{Do you mean similarly?}, human shape information, particularly the boundaries, plays a crucial role in action analysis tasks~\cite{tseng2023edge, chai2022lagrange, pham2022video}. Human shape information can significantly enhance the analysis models' ability to locate different body patterns, thereby improving recognition accuracy. For instance, in 3D reconstruction tasks~\cite{ye2023nef, schmied2023r3d3}, shape information aids in accurately estimating the body structure. Further, in scenarios with complex backgrounds or multiple subjects, boundaries help distinguish between individuals~\cite{he2020bdcn}. Given these considerations, we employ human boundaries to constrain the edges of the flow map \( \boldsymbol{u} \).

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/edge_constraint.pdf}
  \caption{Edge-Chamfer Constraint}
  \label{fig:edge_constraint}
\end{figure}

Edge detection \com{Why all of sudden we start to talk about edge detection?} on visible images has numerous well-established algorithms, such as gradient calculation or the Canny operator. In contrast, defining and extracting edges from a flow map is more challenging. We represent the edges of flow map  \( \boldsymbol{u} \) as a set of discontinuity points \( \boldsymbol{s} \), which can be categorized into intensity and angular discontinuities. Intensity discontinuities occur when the offset between point \(p\) and its neighboring point \(j\) has a substantial difference in magnitude (\( \geq \vartheta_{i} \)), such as between a moving foreground and a static background, which can be represented as:
\begin{equation}
    \boldsymbol{s}_{I} = \left \{ p \in \boldsymbol{u} \mid \left | \boldsymbol{u}_{p} - \boldsymbol{u}_{j} \right |   \ge \vartheta_{i} \right \}.
    \label{eq:intensity_edge}
\end{equation}
On the other hand, angular discontinuities refer to scenarios where the offset between \(p\) and \(j\) exhibits a significant difference in angle (\( \geq \vartheta_{a} \)), typically occurring between different body patterns, which can be represented as:
\begin{equation}
    \boldsymbol{s}_{A} = \left \{ p \in \boldsymbol{u} \mid \frac{\boldsymbol{u}_{p}\cdot \boldsymbol{u}_{j}}{\left | \boldsymbol{u}_{p} \right | \cdot \left | \boldsymbol{u}_{j} \right | } \geq \vartheta_{a} \right \}.
    \label{eq:angular_edge}
\end{equation}
Therefore, for any flow map \( \boldsymbol{u} \), its edge map \( \boldsymbol{s} \) can be formulated by \( \boldsymbol{s}_{I} \cup \boldsymbol{s}_{A} \).

Chamfer distance is often used to measure the distance between two sets of curves. For instance, when measuring the distance between flow edge map \(\boldsymbol{s}\) and human boundaries \(\boldsymbol{e}\), it can be defined as the sum of the nearest distances from any point \(p \in \boldsymbol{s}\) to \(\boldsymbol{e}\). This process can be represented by:
\begin{equation}
    \begin{gathered}
        \mathcal{C}\left( \boldsymbol{s}, \boldsymbol{e} \right) = \sum_{p \in \boldsymbol{s}} \mathcal{D}\left( p, \hat{q} \right), \,
        \text{s.t.} \, \hat{q} = \arg\min_{q \in \boldsymbol{e}} \mathcal{D}\left( p, q \right),
        \label{eq:chamfer_distance}
    \end{gathered}
\end{equation}
where \( \mathcal{D}\left( \cdot \right) \) denotes the Euclidean distance between two points. However, a significant issue is that the operation of finding matching points is inherently discrete. Searching for matching pairs \( \langle p, q \rangle \) between the two dense maps \( \boldsymbol{s} \) and \( \boldsymbol{e} \) requires substantial computation. 

Therefore, we design a method to replace these discrete calculations with matrix operations, namely patch-centroid distance. Based on the concept of calculus, we use kernels with different receptive field sizes to divide both \( \boldsymbol{s} \) and \( \boldsymbol{e} \) into multiple patches across various scales. For any given patch \(\mathcal{P}\), the Chamfer distance between the two curves within that patch (\(\mathcal{P}_{\boldsymbol{s}}\) and \(\mathcal{P}_{\boldsymbol{e}}\)) can be approximated by calculating the distance between the centroids \( \boldsymbol{c} \) of each curve within the patch's boundaries when the point set distribution is smooth. This approximation can be derived through:
\begin{equation}
    \begin{aligned}
        \mathcal{C}\left( \mathcal{P}_{\boldsymbol{s}}, \mathcal{P}_{\boldsymbol{e}} \right) &= \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle }\mathcal{D}\left ( p, \hat{q} \right ) 
        \\ &\approx \mathcal{D}\left ( \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle } p,  \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle } \hat{q} \right ) 
        \\ &\approx \mathcal{D}\left ( \boldsymbol{c}_{\mathcal{P}_{\boldsymbol{s}}}, \boldsymbol{c}_{\mathcal{P}_{\boldsymbol{e}}} \right ) 
        \label{eq:patch_centroid_distance}
    \end{aligned}
\end{equation}
where \(N_p\) denotes the total number of point pairs. Hence, the \( \mathcal{G} \) in \cref{eq:world_constraint} can be further detailed as:
\begin{equation} % \left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right )
    \mathcal{G} = \frac{1}{N_{ms}}\sum_{ms}\left [ \frac{1}{N_{\mathcal{P}}} \sum_{\mathcal{P}\propto ms} \mathcal{C}\left( \mathcal{P}_{\boldsymbol{s}}, \mathcal{P}_{\boldsymbol{e}} \right)  \right ],
    \label{eq:edge_chamfer_constraint}
\end{equation}
where the \(N_{ms}\) and \(N_{\mathcal{P}}\) denotes the depth of multi-scale mechanism and the amount of patches under corresponding scale (\(ms\)), respectively.


\subsection{Dual Coordinate Flow Estimation {\footnotesize \mfinish{Oct.14}}} \label{sec:dual_coord}
\com{This subsection is too wordy and some details can be moved to supplement.}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{asset/network_architecture.pdf}
  \caption{}
  \label{fig:whole_pipeline}
\end{figure*}

By expanding \cref{eq:world_constraint} with the equations derived from \cref{eq:skeleton_muscle_constraint} and \cref{eq:edge_chamfer_constraint}, we can utilize a self-supervised approach to learn the offset of muscle points in the world coordinate system from real-world scenarios, which corresponds to the concept of World Flow (\( \boldsymbol{u_w} \)) introduced in \cref{sec:problem_formulation}. In some action analysis tasks, in fact, from a human point of view, they rely more on analyzing the internal motion than on the interaction between the human body and the scene, such as analyzing the gait of a pedestrian or the diving process of an athlete. Therefore, we introduce the concept of Local Flow (\( \boldsymbol{u_l} \)) to better capture these potential motion states. Together with World Flow, our Dual Coord. Flow allow the analysis model to think in the same way as the human kinematic analysis process, providing a novel possibility for the establishment of the world model \com{This is not clear to me. Why all of a sudden we are talking about world model?}.

In \cref{eq:dual_coord_flow}, we discussed the relationship between \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \). To obtain both of them, which together from our Dual Coord. Flow,
we avoid using two flow estimation network \(\Phi\) independently to estimate \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \). Instead, we leverage the principle of vector decomposition. By using a single flow estimation network \(\Phi\) to estimate \( \boldsymbol{u_w} \), and a shallow network \(\Psi\) to estimate \( \boldsymbol{u_s} \), we indirectly solve for \( \boldsymbol{u_l} \). This approach significantly reduces the computational load during both training and inference, this process can be formulated by:
\begin{equation}
    \begin{aligned}
        \Phi \left( \omega_{1}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) &\Rightarrow \boldsymbol{u_w},
        \\ \Psi \left( \omega_{2}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}, \boldsymbol{u_w} \right) &\Rightarrow \boldsymbol{u_s},
        \\ \boldsymbol{u_w} - \boldsymbol{u_s} &= \boldsymbol{u_l}.
    \end{aligned}
\end{equation}
\com{Why not uw=phi()?}

Since we use different reference systems, \cref{eq:world_constraint}, which constrains \( \boldsymbol{u_w} \), requires transformations to be applicable for constraining \( \boldsymbol{u_l} \) \com{grammar error}. Specifically, this transformation affects \( \vec{\boldsymbol{k}} \) in \cref{eq:skeleton_muscle_constraint}. In \cref{sec:joint_constraint}, \( \vec{\boldsymbol{k}} \) represents the offsets between two skeletal maps (\( \boldsymbol{k}_t \) and \(\boldsymbol{k}_{t+1} \)), which is defined with respect to the ground. Therefore, we need to convert this displacement to be relative to the subject itself, which can be achieved by aligning \( \boldsymbol{k}_t \) and \( \boldsymbol{k}_{t+1} \). We propose two alignment methods to achieve this. The first is homography-based matching, which calculates a transformation matrix to minimize the overall offsets between \( \boldsymbol{k}_t \) and \( \boldsymbol{k}_{t+1} \) through an analytical solution. By applying this transformation to \( \boldsymbol{k}_{t+1} \), alignment with \( \boldsymbol{k}_t \) can be accomplished, which proves effective in most scenarios \com{better mention which result supports this claim}. However, for some specific tasks such as analyzing diving sequences, where rotational motion is dominant, the homography-based matching may lead to skeletal distortions. For these cases, we design a head-aligned based alignment approach. In this method, \( \boldsymbol{k}_{t+1} \) is rotated to align its head keypoints as closely as possible with those of \( \boldsymbol{k}_t \). After applying either of these two alignment methods, we obtain adjusted skeletal map \( \boldsymbol{k}_{t+1}' \), from which we derive the subject-relative offsets \( \vec{\boldsymbol{k}'} \). Based on this, we transfer \( \mathcal{F} \) to \( \mathcal{F}'\) \com{Need to say their names to save reviewers effort}. Thus, similar to \cref{eq:world_constraint}, the constraint for \( \boldsymbol{u_l} \) can be represented as:
\begin{equation}
    \boldsymbol{u_l} =  \arg\min_{\boldsymbol{u}}\left [ \mathcal{F}'\left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + \alpha \cdot \mathcal{G}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right ) \right ]. \label{eq:local_constraint}
\end{equation}
\com{It seems that Eq. 12 also computes ul. Then what is the relationship between Eq. 12 and 13?}
Based on \cref{eq:world_constraint} and \cref{eq:local_constraint}, we can determine the optimal values for \( \omega_{1} \) in \( \Phi \) and \( \omega_{2} \) in \( \Psi \) by applying the chain rule of differentiation.




==> section/03_method_v3.tex <==
\section{Methodology {\small \mfinish{Nov.04} \TODO{Updating}}}

\TODO{Variable Table}

\subsection{Problem Formulation} \label{sec:problem_formulation}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/whole_pipeline.pdf}
  \caption{Problem Formulation of Our Joint Constraint Learning Framework: Introducing pose and shape information to construct an accurate human motion representation.} 
  \label{fig:joint_constraint} % Just a schematic diagram. I will replace it with a formal one after the meeting.
\end{figure}

To learn human-centric motion representations from real-world scenarios, which contain detailed human motion and shape information, \methodName{} introduces a Joint Constraint framework that captures the offsets of each human body point between consecutive frames. 
Given a pair of consecutive frames \( \left( \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) \), \methodName{} estimates human motion relevant to the external environment, referred to as the World Flow \( \left( \boldsymbol{u_w} \right) \).

Specifically, using a flow estimation network \( \Phi \), various types of flow maps can be computed by \(\boldsymbol{u} = \Phi \left( \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}; \omega_{1} \right)\) where \( \omega_{1} \) represents the network parameters. A common solution within \( \boldsymbol{u} \) is the widely used Optical Flow, which often relies on supervised learning with object-centric datasets. In contrast, for human-centric scenarios, we focus on capturing human-specific motion information in \( \boldsymbol{u_w} \), filtering out non-human motion to provide more accurate human movement data than standard optical flow.

To achieve this, we introduce our Joint Constraint learning framework, which includes two fidelity terms: the skeletal constraint \( \mathcal{F} \) and the boundary constraint \( \mathcal{G} \). 
The skeletal constraint ensures that our flow captures precise human motion by utilizing pose information, which enforces that each body point’s movement adheres to realistic physiological constraints, such as coordinated skeletal and body movements. Specifically, \( \mathcal{F} \) quantifies the discrepancy between the estimated \( \boldsymbol{u} \) and the pose offset from \(\boldsymbol{x}_{t}\) to \(\boldsymbol{x}_{t+1}\). Additionally, to incorporate human shape and fine-grained motion, we employ the boundary constraint, which aligns human shapes in the flow map and frames by measuring the chamfer distance between the boundaries of humans in \( \boldsymbol{u} \) and \( \boldsymbol{x}_{t} \). Therefore, our target world flow \( \boldsymbol{u_w} \) is thus defined as:
\begin{equation}
    \boldsymbol{u_w} =  \arg\min_{\boldsymbol{u}}\left [ \mathcal{F}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + \alpha \cdot \mathcal{G}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right ) \right ], \label{eq:joint_constraint}
\end{equation}
where \( \alpha \) is a weighting factor that balances the contributions of each term. The specific implementations of \( \mathcal{F} \) and \( \mathcal{G} \) will be discussed in \cref{sec:joint_constraint}.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{asset/wl_flows.pdf}
  \caption{Definition of World-Local Flows: The distinction and correlation between world motion and local motion. Using subject motion as a bridge, they can be converted through vector composition and decomposition.}
  \label{fig:wl_flows}
\end{figure}

In certain tasks that focus specifically on analyzing human motion, \eg re-identification based on gait or scoring an athlete's diving performance, the motion relative to the environment holds less significance. Analysis for these tasks should instead be based on motion relative to the subject itself. For example, examining how the arm has moved compared to the previous moment. We refer to this motion as Local Flow \( \left( \boldsymbol{u_l} \right) \).

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{asset/skeletal_constraint_full.pdf}
  \caption{Two Components of Skeletal Constraint: (a) the process of matching any point \(p\) on the body to its corresponding point \(\hat{q}\) on the skeleton; (b) an angular sub-constraint to ensure estimated motion aligns closely with the skeleton's movement direction; and (c) an intensity constraint to maintain consistency in motion magnitude between estimated motion and skeleton's movement.}
  \label{fig:skeleton_constraint}
\end{figure*}

Inspired by Galilean transformations in physical kinematics, we identify an underlying connection between \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \), as illustrated in \cref{fig:wl_flows}. As a result, we can avoid using a completely separate network \( \Phi' \) to estimate \( \boldsymbol{u_l} \). Instead, we use a lightweight network \( \Psi \) to estimate the overall motion trend of the subject \( \left( \boldsymbol{u_s} \right) \) based on \( \boldsymbol{u_w} \). By applying vector decomposition, we can indirectly estimate \( \boldsymbol{u_l} \) with reduced computational cost, denoted as:
\begin{equation}
    \begin{gathered}
        \boldsymbol{u_s} = \Psi \left(\boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}, \boldsymbol{u_w}; \omega_{2} \right), \\
        \boldsymbol{u_l} = \boldsymbol{u_w} - \boldsymbol{u_s},
    \end{gathered}
    \label{eq:wl_flow}
\end{equation}
where \( \omega_{2} \) represents the network parameters. Similarly, our joint constraint learning framework also applies to \( \boldsymbol{u_s} \), as detailed in \cref{sec:wl_flow}

\subsection{Joint Constraint Learning Framework {\footnotesize \mfinish{Nov.04}}} \label{sec:joint_constraint}

In our proposed learning framework, as formulated in \cref{eq:joint_constraint}, we define two regularization terms. The skeletal constraint \( \mathcal{F} \) establishes the general range of motion, while the boundary constraint \( \mathcal{G} \) refines motion details and incorporates shape information. Both terms involve a number of discrete operations. In this subsection, we discuss these constraints in detail and explain how we transform these discrete operations into differentiable matrix computations.

\vspace{4pt}
\noindent\textbf{\textit{(a) Skeletal Constraint:}} {\footnotesize \mfinish{Nov.04} \TODO{Ready for Comment}}
In action analysis tasks, accurate motion information is essential. It directly impacts the model's ability to recognize specific patterns. This is especially important in cases involving complex or subtle motion dynamics. Pose, \ie skeletal offsets, provide valuable insights for capturing detailed kinematic information.\com{This paragraph is redundant and can be deleted. We should briefly describe the key idea.}

Instead of constructing pseudo ground truth based on pose offsets like PoseFlow~\cite{zhang2018poseflow}, we establish a dynamic relationship between skeleton and body points. This approach reduces the influence of errors from pose estimation while allowing us to preserve more shape information. Thereby creating a kinematic fidelity constraint on our flow learning process. Specifically, our process begins with 2D pose estimation, \eg ED-Pose~\cite{yang2022explicit}, which extract joint points \( \mathbb{R}^{17 \times 3} \) \com{what is that? We need to explain it captures data of 17 joints in 3-dim space.} from frame \( \boldsymbol{x}_t \). We then use interpolation to construct a skeleton map with confidence values \( \boldsymbol{k}_{t} \in \mathbb{R}^{N_{k} \times 3} \) \com{what is the meaning of confidence values}. Each bone segment is uniformly sampled, typically consisting more than \(200\) points (\( N_{k} \geq 200 \)).

As illustrated in ~\cref{fig:skeleton_constraint} \com{should be referred to as Fig 4(a)}, for any body point \( p \in \boldsymbol{u} \) \com{why p in u? Shouldn't we say p on the flow map u?} (red point), we identify the closest keypoint \( \hat{q} \) (blue point) on the skeleton map by minimizing a weighted distance. \com{We need to briefly describe the idea instead of having reviewers to figure out the idea from the equation.} This process is defined as:
\begin{equation}
    \hat{q} = \arg\min_{q \in \boldsymbol{k}_{t} \cdot s} \left( \left\| p - q \right\| * -{v}_{q}\right), ~\ \mathit{s.t.} ~ p \in \boldsymbol{u} \cdot s, 
    \label{eq:skeleton_match}
\end{equation}
where \( v_{q} \) represents the visibility and confidence of the point \( q \) \com{how did you get vq? Also, what is "-" before vq}. The \( \cdot s \) operation restricts matching to the region occupied by subject \( s \), thus preventing incorrect voxel matches in \( \boldsymbol{u} \) in multi-person scenarios. Typically, \( \hat{q} \) is the point on the skeleton segment nearest to \( p \), found by perpendicular projection.

\com{Why not use a label to indicate this is for an angular constraint?}
Through this skeleton-body points matching, we construct a dynamic constraint. Based on human biological priors \com{kinematic constraint?}, we infer that for any body point \( p \), its movement direction will not be orthogonal to that of its corresponding skeletal points \( \hat{q} \), nor will it differ significantly in motion intensity. Thus, we define a skeletal constraint that includes angular and intensity sub-constraints to create a kinematic term for each \( \left \langle p - \hat{q} \right \rangle  \) pair.

\com{Is this paragraph to implement the idea described above? The transition is not clear.}
As shown in ~\cref{fig:skeleton_constraint} \com{(b)}, we calculate the angle formed between the motion vector of the body point \( \boldsymbol{u}_{p} \) (red vector) and that of the skeletal point \( \vec{\boldsymbol{k}}_{\hat{q}} \) (blue vector) \com{Is k the skeleton map? Then why here k is the motion vector?}. Using a \com{manually specified?} threshold \( \vartheta_{a} \), we establish ranges for the ideal (green sector) and excessive (red sector) motion. Thus, the angular sub-constraint can be formulated as:
\begin{equation}
    \mathcal{F}_{A}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) = \mathbb{I}\left ( \frac{\boldsymbol{u}_{p}\cdot \vec{\boldsymbol{k}}_{\hat{q}}}{\left | \boldsymbol{u}_{p} \right | \cdot \left | \vec{\boldsymbol{k}}_{\hat{q}} \right | } \geq \vartheta_{a} \right ),
    \label{eq:angular_constraint}
\end{equation}
where \( \vec{\boldsymbol{k}} \in \mathbb{R}^{n_{k} \times 3} \) represents the offset between two skeletal maps, calculated as \( \boldsymbol{k}_{t} - \boldsymbol{k}_{t+1} \). The term \( \mathbb{I} \left( \cdot \right) \) is an indicator function used to count body points with abnormal motion.

\com{Why not use a label to indicate this is for an intensity constraint?}
Similarly, we expect the motion intensity of a body point and its corresponding skeletal point to be consistent. To define acceptable and error ranges for the intensity of \( \boldsymbol{u}_{p} \), we use \( \left( \vartheta_{i}^{l}, \vartheta_{i}^{h} \right) \) and \( \vec{\boldsymbol{k}}_{\hat{q}} \). The acceptable range is represented by a green ring, while errors are indicated by a red circle (low intensity) and a red ring (high intensity). When \( \boldsymbol{u}_{p} \) falls outside the green ring, a penalty value is applied as a constraint. This can be formulated as:
\begin{equation}
    \mathcal{F}_{I}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) = \operatorname{ReLU}\left[\left(\boldsymbol{u}_{p}-\vartheta_{i}^{l} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right) \cdot\left(\boldsymbol{u}_{p}-\vartheta_{i}^{h} \cdot \vec{\boldsymbol{k}}_{\hat{q}}\right)\right].
    \label{eq:intensity_constraint}
\end{equation}

With the dynamic sub-constraints on both angular and intensity, we can effectively bind the motion of body points to skeletal motion. It precisely defines the possible range of movement for each point on the human body. Thus skeletal constraint \( \mathcal{F} \) in \cref{eq:joint_constraint} can be further detailed as:
\begin{equation}
    \mathcal{F} = \frac{1}{h \cdot w} \sum_{p \in \boldsymbol{u}} \left[ \mathcal{F}_{A}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) + \beta \cdot \mathcal{F}_{I}\left ( \boldsymbol{u}_{p}, \vec{\boldsymbol{k}}_{\hat{q}} \right ) \right ],
    \label{eq:skeletal_constraint}
\end{equation}
where \( \beta \) balances the two sub-constraints.


\vspace{4pt}
\noindent\textbf{\textit{(b) Boundary Constraint:}}
Human shape information, \ie the boundaries, plays an important role in action analysis tasks~\cite{tseng2023edge, chai2022lagrange, pham2022video}. It can significantly enhance a model's ability to identify various body patterns, thereby improving pattern recognition accuracy. For example, in gait recognition tasks, shape information helps accurately estimate body structure. Additionally, in scenarios with complex backgrounds or multiple subjects, boundaries aid in distinguishing individuals~\cite{he2020bdcn}. Given these considerations, we use human boundaries \( \boldsymbol{e} \) to constrain the edge of the flow map \( \boldsymbol{s} \).

Specifically, inspired by point cloud matching~\cite{} and medical image segmentation~\cite{}, we use the Chamfer distance to measure the distance between \( \boldsymbol{e} \) and \( \boldsymbol{s} \) \com{the names of the symbols are needed}. It is defined as the sum of the nearest distances from each point \( p \in \boldsymbol{s} \) to \com{on the flow map s} \( \boldsymbol{e} \). This process can be represented by:
\begin{equation}
    \begin{gathered}
        \mathcal{C}\left( \boldsymbol{s}, \boldsymbol{e} \right) = \sum_{p \in \boldsymbol{s}} \mathcal{D}\left( p, \hat{q} \right), \,
        \text{s.t.} \, \hat{q} = \arg\min_{q \in \boldsymbol{e}} \mathcal{D}\left( p, q \right),
        \label{eq:chamfer_distance}
    \end{gathered}
\end{equation}
where \( \mathcal{D}\left( \cdot \right) \) represents the Euclidean distance between two points.

However, searching for matching pairs \( \langle p, q \rangle \) between the two dense curves \( \boldsymbol{s} \) and \( \boldsymbol{e} \) demands substantial computation. To efficiently measure the distance between them, we design a method that replaces discrete calculations with matrix operations, termed patch-centroid distance. Leveraging concepts from calculus, we use kernels with various receptive field sizes to divide both \( \boldsymbol{s} \) and \( \boldsymbol{e} \) into multiple patches at different scales. For any given patch \(\mathcal{P}\), the Chamfer distance between the curves within that patch (\(\mathcal{P}_{\boldsymbol{s}}\) and \(\mathcal{P}_{\boldsymbol{e}}\)) can be approximated by calculating the distance between the centroids \( \boldsymbol{c} \) of each curve within the patch, assuming a smooth distribution of points. This approximation can be expressed as:
\begin{equation}
    \begin{aligned}
        \mathcal{C}\left( \mathcal{P}_{\boldsymbol{s}}, \mathcal{P}_{\boldsymbol{e}} \right) &= \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle }\mathcal{D}\left ( p, \hat{q} \right ) 
        \\ &\approx \mathcal{D}\left ( \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle } p,  \frac{1}{N_p}\sum_{\left \langle p, \hat{q} \right \rangle } \hat{q} \right ) 
        \\ &\approx \mathcal{D}\left ( \boldsymbol{c}_{\mathcal{P}_{\boldsymbol{s}}}, \boldsymbol{c}_{\mathcal{P}_{\boldsymbol{e}}} \right ) 
        \label{eq:patch_centroid_distance}
    \end{aligned}
\end{equation}
where \(N_p\) denotes the total number of point pairs.

Furthermore, we can increase the accuracy of this approximation by further dividing patches and calculating at additional scales. Thus boundary constraint \( \mathcal{G} \) in \cref{eq:joint_constraint} can be represented as:
\begin{equation}
    \mathcal{G} = \frac{1}{N_{ms}}\sum_{ms}\left [ \frac{1}{N_{\mathcal{P}}} \sum_{\mathcal{P}\propto ms} \mathcal{C}\left( \mathcal{P}_{\boldsymbol{s}}, \mathcal{P}_{\boldsymbol{e}} \right)  \right ],
    \label{eq:edge_chamfer_constraint}
\end{equation}
where \(N_{ms}\) denotes the depth of the multi-scale mechanism, and \(N_{\mathcal{P}}\) denotes the number of patches at scale \(ms\).

\subsection{World-Local Flow Estimation {\footnotesize \mfinish{Oct.14}}} \label{sec:wl_flow}
{\small \TODO{Will Ready by Nov.4 Noon}}
\com{This subsection is too wordy and some details can be moved to supplement.}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth, height=0.2\textheight]{asset/network_architecture.pdf}
  \caption{}
  \label{fig:whole_pipeline}
\end{figure*}

By expanding \cref{eq:world_constraint} with the equations derived from \cref{eq:skeleton_muscle_constraint} and \cref{eq:edge_chamfer_constraint}, we can utilize a self-supervised approach to learn the offset of muscle points in the world coordinate system from real-world scenarios, which corresponds to the concept of World Flow (\( \boldsymbol{u_w} \)) introduced in \cref{sec:problem_formulation}. In some action analysis tasks, in fact, from a human point of view, they rely more on analyzing the internal motion than on the interaction between the human body and the scene, such as analyzing the gait of a pedestrian or the diving process of an athlete. Therefore, we introduce the concept of Local Flow (\( \boldsymbol{u_l} \)) to better capture these potential motion states. Together with World Flow, our Dual Coord. Flow allow the analysis model to think in the same way as the human kinematic analysis process, providing a novel possibility for the establishment of the world model \com{This is not clear to me. Why all of a sudden we are talking about world model?}.

In \cref{eq:dual_coord_flow}, we discussed the relationship between \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \). To obtain both of them, which together from our Dual Coord. Flow,
we avoid using two flow estimation network \(\Phi\) independently to estimate \( \boldsymbol{u_w} \) and \( \boldsymbol{u_l} \). Instead, we leverage the principle of vector decomposition. By using a single flow estimation network \(\Phi\) to estimate \( \boldsymbol{u_w} \), and a shallow network \(\Psi\) to estimate \( \boldsymbol{u_s} \), we indirectly solve for \( \boldsymbol{u_l} \). This approach significantly reduces the computational load during both training and inference, this process can be formulated by:
\begin{equation}
    \begin{aligned}
        \Phi \left( \omega_{1}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right) &\Rightarrow \boldsymbol{u_w},
        \\ \Psi \left( \omega_{2}; \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1}, \boldsymbol{u_w} \right) &\Rightarrow \boldsymbol{u_s},
        \\ \boldsymbol{u_w} - \boldsymbol{u_s} &= \boldsymbol{u_l}.
    \end{aligned}
\end{equation}
\com{Why not uw=phi()?}

Since we use different reference systems, \cref{eq:world_constraint}, which constrains \( \boldsymbol{u_w} \), requires transformations to be applicable for constraining \( \boldsymbol{u_l} \) \com{grammar error}. Specifically, this transformation affects \( \vec{\boldsymbol{k}} \) in \cref{eq:skeleton_muscle_constraint}. In \cref{sec:joint_constraint}, \( \vec{\boldsymbol{k}} \) represents the offsets between two skeletal maps (\( \boldsymbol{k}_t \) and \(\boldsymbol{k}_{t+1} \)), which is defined with respect to the ground. Therefore, we need to convert this displacement to be relative to the subject itself, which can be achieved by aligning \( \boldsymbol{k}_t \) and \( \boldsymbol{k}_{t+1} \). We propose two alignment methods to achieve this. The first is homography-based matching, which calculates a transformation matrix to minimize the overall offsets between \( \boldsymbol{k}_t \) and \( \boldsymbol{k}_{t+1} \) through an analytical solution. By applying this transformation to \( \boldsymbol{k}_{t+1} \), alignment with \( \boldsymbol{k}_t \) can be accomplished, which proves effective in most scenarios \com{better mention which result supports this claim}. However, for some specific tasks such as analyzing diving sequences, where rotational motion is dominant, the homography-based matching may lead to skeletal distortions. For these cases, we design a head-aligned based alignment approach. In this method, \( \boldsymbol{k}_{t+1} \) is rotated to align its head keypoints as closely as possible with those of \( \boldsymbol{k}_t \). After applying either of these two alignment methods, we obtain adjusted skeletal map \( \boldsymbol{k}_{t+1}' \), from which we derive the subject-relative offsets \( \vec{\boldsymbol{k}'} \). Based on this, we transfer \( \mathcal{F} \) to \( \mathcal{F}'\) \com{Need to say their names to save reviewers effort}. Thus, similar to \cref{eq:world_constraint}, the constraint for \( \boldsymbol{u_l} \) can be represented as:
\begin{equation}
    \boldsymbol{u_l} =  \arg\min_{\boldsymbol{u}}\left [ \mathcal{F}'\left ( \boldsymbol{u}, \boldsymbol{x}_{t}, \boldsymbol{x}_{t+1} \right ) + \alpha \cdot \mathcal{G}\left ( \boldsymbol{u}, \boldsymbol{x}_{t}\right ) \right ]. \label{eq:local_constraint}
\end{equation}
\com{It seems that Eq. 12 also computes ul. Then what is the relationship between Eq. 12 and 13?}
Based on \cref{eq:world_constraint} and \cref{eq:local_constraint}, we can determine the optimal values for \( \omega_{1} \) in \( \Phi \) and \( \omega_{2} \) in \( \Psi \) by applying the chain rule of differentiation.




==> section/04_exp_v1.tex <==
\section{Experiments {\small \TODO{Need Update}}}

%
% NeuIPS version
%
% To validate the effectiveness of our proposed HuMoR across a range of action analysis tasks, as outlined in Eq.~\ref{eq:analysis_paradigm}, we conduct experiments on three representative tasks: CASIA-B for gait recognition, Diving48 for sports recognition, and MHAD for video prediction. 
% To benchmark our method's performance, we compare it with six well-established optical flow estimation algorithms, including RAFT\cite{teed2020raft}, GMA\cite{jiang2021learning}, GMFlow\cite{xu2022gmflow}, CRAFT\cite{sui2022craft}, SKFlow\cite{sun2022skflow}, VideoFlow\cite{shi2023videoflow} and FlowFormer{\scriptsize{++}}\cite{shi2023flowformer++}. 
% To ensure the fairness of comparisons, each experiment is conducted after fine-tuning both the optical flow estimator and task-specific models on the training sets dedicated to each task, using consistent hyper-parameters. 
% The additional input modalities \(v\) specified in Eq.~\ref{eq:analysis_paradigm} are configured as silhouettes for gait recognition and RGB frames for sports recognition and video prediction.

To demonstrate the widespread advantages of HuMoR in human-centric action analysis tasks, we choose three representative tasks: gait recognition, which requires learning subtle differences from periodic movements; action recognition, which demands accurate capture of human motion within short temporal intervals; and video generation, which necessitates precise motion information for constraining future frame generation. To emphasize the impact of motion information and minimize the overshadowing effects of other modalities, we carefully choose prototype base-models for each task, i.e., GaitSet~\cite{chao2021gaitset} for gait recognition, TSN~\cite{wang2016temporal} for action recognition, and LGC-VD~\cite{yang2023video} for video generation. This allows us to precisely assess the differences brought about by every motion information across various tasks. All experiments are conducted on 8 NVIDIA A6000 GPUs.

% \input{tabular/full-action}

\subsection{Results}

\begin{table*}[t]
  \centering
  \input{table/quantitative_aug}
  \TODO{Need Update with latest results.}
  % \includegraphics[width=0.98\textwidth，height=0.3\textheight]{assets/preview.pdf}
  \caption{}
  \label{tab:quantitative}
\end{table*}

% In our analysis of the impact of our proposed HuMoR on gait recognition, we utilized the widely recognized CASIA-B dataset\cite{zheng2011robust}. 
To validate the precision of HuMoR compared to optical flow in scenarios with stable backgrounds, we conducted comparative experiments on the CASIA-B dataset~\cite{zheng2011robust}, which includes videos of 124 subjects under three distinct walking conditions (normal walking, wearing a coat, and carrying a bag) captured from 11 view angles.
As shown in the first three columns in Tab.~\ref{tab:bio-action}, introducing motion information significantly enhances accuracy. 
Both the use of optical flow \(\mathbf{u}^\mathsf{opt}\) and our HuMoR \(\mathbf{u^{*}}\) as \(u\) in \(\Psi_{G}\left( \mathbf{u}, \mathbf{v} \right)\) outperform the baseline model \(\Psi_{G}\left( \mathbf{v} \right)\), which only utilizes silhouettes. 
Notably, employing a single modality of HuMoR, either \(\mathbf{u^{w}}\) or \(\mathbf{u^{l}}\), results in further improvements; for instance, the Rank-1 accuracy on the CMC curve under normal walking conditions (Col.~{\footnotesize NM@R1}) increases by 4.41\%. These enhancements are even more pronounced in challenging conditions such as walking with a bag (Col.~{\footnotesize BG@R1}) and with a coat (Col.~{\footnotesize CL@R1}), with gains of 11.09\% and 10.07\%, respectively. These significant improvements underscore the substantial role that accurately estimated motion information by HuMoR can play, even when using a recognizer with a smaller parameters such as GaitSet.
Crucially, when both modalities of HuMoR, \(\{ \mathbf{u^{w}}, \mathbf{u^{l}} \}\), are employed as \(\mathbf{u}\), these impressive gains are further amplified (Row.~{\footnotesize HuMoR} {\tiny W.+L.}), further validate the our hypothesis that integrating multiple coordinate system into the analysis can enhance the learning accuracy of recognition models.
% benefiting from our dual-coordinate system representation approach, as detailed in Eq.~\ref{eq:multi_coordinate} and Eq.~\ref{eq:coord_transfer}.

\subsection{Results on Action Recognition}

% \begin{figure}[t]
%   \centering
%   \includegraphics[trim=0 0 0 0,clip,width=\textwidth]{assets/qualitative.png}
%   \caption{Visualizations of the predicted motion among different methods on CASIA-B. Significant differences are highlighted with red arrows, showcasing the distinct advantages of HuMoR.}
%   % : more accurate edge delineations with W. and unique motion information with L.} 
%   \label{fig:qualitative}
%   \vspace{-12pt}
% \end{figure}

%Action recognition, a fundamental task in computer vision, entails identifying and classifying various human activities within video sequences. This capability is pivotal for applications ranging from surveillance systems to interactive gaming. 
% To assess the efficacy of our %Human-centric Motion Representation (
% HuMoR in action recognition, we conduct experiments on the Diving48 dataset \cite{li2018resound}, which comprises approximately 18,000 finely trimmed clips of 48 distinct and well-defined dive sequences. For  video classification, we employ the TSN\cite{wang2016temporal} as the classifier \(\Psi_{S}\), with RGB frames as the additional input modalities \(\mathbf{v}\). 
% Quantitative comparisons illustrating the performance of our approach compared to existing methods are presented in the middle two columns of Tab.~\ref{tab:bio-action}.
% TODO: analysis of results
To address HuMoR's accuracy in representing high-speed motions at low resolutions, we seletec Diving48~\cite{li2018resound} as the benchmark for action recognition. This dataset includes approximately 18,000 finely trimmed clips of 48 distinct and well-defined dive sequences. Diving movements are typically completed within 2 seconds and are characterized by high speeds, often resulting in considerable motion blur. Additionally, the camera movement is synchronized with the diver's position to keep the subject centrally framed, further challenging our dual-coordinate precision metrics. As indicated in Col.~{\footnotesize \{Acc@1 \& Acc@5\}}, employing HuMoR leads to higher accuracy (1.67\%). Notably, while \(\mathbf{u^l}\) achieves higher accuracy at Acc@1, it slightly under-performs compared to \(\mathbf{u^w}\) at Acc@5, highlighting the difference between these two modalities: motion representation in world-coordinate, including optical flow and \(\mathbf{u^w}\), prompt the model to learn from broader movement trends (e.g., the overall downward trajectory during a dive), whereas local-coordinate, by eliminating overarching motion trends, encourage the model learning from tiny motion details (e.g., specific limb movements), thereby giving \(\mathbf{u^l}\) an advantage in precise judgements, whereas \(\mathbf{u^w}\) excels in general estimations.

\subsection{Results on Video Generation}

% \input{tabular/prediction}

As a challenging task in computer vision, video generation involves creating a sequence of images from a given initial frame and specified conditions. 
The accuracy of motion information is particularly critical for fine-grained generation, which accesses our HuMoR's ability to precisely represent significant human movements such as waving hands of squatting. For this purpose, we conducted comparative experiments on the MHAD dataset\cite{chen2015utd} against other optical flow methods.
Given the global coordinates of subjects are fixed in this dataset, we specifically evaluated our \(\mathbf{u^l}\).
Compared to optical flow algorithms, the generation model based on HuMoR results in higher Structural Similarity (Col.~{\footnotesize SSIM} {\footnotesize (0.25\%\(\uparrow\))}) and substantially improve the Frechet Video Distance (Col.~{\footnotesize FVD} {\footnotesize (59.28\%\(\uparrow\))}), which are crucial for assessing the quality of generated videos. These results confirm that HuMoR can accurately represent not only cyclic (as in gait) and rapid (as in diving) motion, but also significant ones, showcasing its broad applicability across various motion-intensive tasks.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{asset/video_generation.pdf}
  \caption{}
  \label{fig:video_generation}
\end{figure*}

\subsection{Qualitative Experiments}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{asset/qualitative_comparison.pdf}
  \caption{}
  \label{fig:qualitative_comparison}
\end{figure*}

In Fig.~\ref{fig:qualitative_comparison}, we display the qualitative results of HuMoR's dual modalities on the CASIA dataset, illustrating the distinctions between HuMoR and optical flow methods. The highlighted regions underscore the benefits of our approach; kinematic constraints enable the precise quantification of motion magnitude, as evidenced when compared to Col.~{\footnotesize 1}. Similarly, the application of semantic constraints enhances the clarity and accuracy of edge representation, as indicated by the red arrows in Col.~{\footnotesize 2}. Additionally, we showcase the differences between HuMoR's local-coordinate representation (HuMoR {\scriptsize L.} \(\mathbf{u^l}\)) and the combination of global-coordinate measures (HuMoR {\scriptsize W.} \(\mathbf{u^w}\) with optical flow methods), elucidating how each modality contributes to comprehensive motion analysis.

\subsection{Ablation Studies}

% \begin{table}[t]
%   \centering
%   \begin{tikzpicture}
%         \draw[gray, thick] (0,0) rectangle (0.48\textwidth, 0.2\textheight);
%         \node at (0.24\textwidth, 0.1\textheight) {Ablation Placeholder.};
%   \end{tikzpicture}
%   \TODO{Ablation Study}
%   % \includegraphics[width=0.98\textwidth，height=0.3\textheight]{assets/preview.pdf}
%   \caption{Ablation Study}
%   \label{tab:ablation}
% \end{table}

% \begin{figure*}[t]
%   \centering
%   \input{table/ablation_aug}
%   \label{tab:ablation}
% \end{figure*}

We conduct a series of ablation studies to investigate the distinct effects of the two constraints utilized in HuMoR. Fig.~\ref{fig:ablation} demonstrates the difference when each constraint is applied individually. Employing only the semantic constraint \(g_s\) leads to accurate human edges but results in significant deviations in the direction and magnitude of motion. Conversely, using solely the kinematic constraint \(g_k\) generally aligns motion information correctly concerning direction and magnitude. However, similar to some early optical flow estimation algorithms, which potentially lead to unintended motion information. As shown in the figure, combining both constraints yields a motion representation that accurately captures both precise edges and accurate motion information, effectively optimizing the representation for human-centric motion analysis.

==> table/ablation_algorithm.tex <==
\centering
\resizebox{0.48\textwidth}{!}{
    \small
    \begin{tabular}{lccccc} 
    \toprule
    Algorithms & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\) & {Acc@1}\(\uparrow\)    & {Acc@5}\(\uparrow\)
    \\
    \midrule
    Boundary: Canny w/o Smoothing              &                   &                   &                   \\
    Boundary: EDTER                            &                   &                   &                   \\ 
    \midrule
    Pose: AlphaPose                            &                   &                   &                   \\ 
    \midrule
    Segmentation: DINOv2                       &                   &                   &                   \\ 
    \midrule
    Recognition: Pretrained MotionBERT         &                   &                   &                   \\ 
    Recognition: SMPL from MotionBERT          &                   &                   &                   \\ 
    Recognition: SHOF                          &                   &                   &                   \\ 
    Recognition: MHOF                          &                   &                   &                   \\ 
    \midrule
    \methodName{} {\scriptsize [Canny + ED-Pose + U\(^2\)Net]}                      & 98.26    & 95.62    & 87.66    & 72.99    & 97.62    \\
    \methodName{}{\scriptsize+} {\scriptsize [Pretrained on subset Human3.6M]}      &          &          &          &          &          \\ 
    \bottomrule
    \end{tabular}
}

==> table/ablation_angular.tex <==
\centering
\resizebox{0.45\textwidth}{!}{
    \small
    \begin{tabular}{lccc} 
    \toprule
    \(\vartheta_{a}\) & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\)
    \\
    \midrule
    \(5^\circ\)              & 96.31             & 94.12             & 84.98             \\
    \rowcolor{mint}
    \(15^\circ\)             & 98.26             & 95.62             & 87.66             \\
    \(25^\circ\)             & 98.21             & 95.27             & 87.92             \\ 
    \(35^\circ\)             & 97.71             & 94.87             & 85.33             \\ 
    \(45^\circ\)             & 94.80             & 92.20             & 80.19             \\ 
    \bottomrule
    \end{tabular}
}

==> table/ablation_canny.tex <==
\centering
\resizebox{0.45\textwidth}{!}{
    \small
    \begin{tabular}{lccc} 
    \toprule
    Edge Det. & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\)
    \\
    \midrule
    Canny w/o Smoothing              & 97.21             & 95.82             & 87.49             \\
    \rowcolor{mint}
    Canny with Smoothing             & 98.26             & 95.62             & 87.66             \\
    EDTER                            & 97.71             & 94.98             & 87.81             \\ 
    \bottomrule
    \end{tabular}
}

==> table/ablation_v1.tex <==
\begin{minipage}[c]{\textwidth}
    % \centering
    \raggedright
    \begin{tabular}{>{\centering\arraybackslash}p{18pt} >{\centering\arraybackslash}p{18pt} cccccc}
        \toprule
        \multicolumn{2}{c}{\textbf{Constraint}}        
        & \multicolumn{3}{c}{\textbf{Gait Rec. \scriptsize{(CASIA-B)}}}
        & \multicolumn{2}{c}{\textbf{Action Rec. \scriptsize{(Diving48)}}}
        \\
        \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7}
        \textbf{\(g_s\)} & \textbf{\(g_k\)}
        & {\small\textbf{NM}\(\uparrow\)} & {\small\textbf{BG}\(\uparrow\)} & {\small\textbf{CL}\(\uparrow\)}
        & {\small\textbf{Acc{\scriptsize@R1}}\(\uparrow\)}    & {\small\textbf{Acc{\scriptsize@R5}}\(\uparrow\)}
        \\
        \midrule
        \checkmark &                & 96.99             & \uline{93.09}     & \uline{84.93}     & 68.17     & 95.23 \\
        & \checkmark                & \uline{97.15}     & 91.47             & 83.01             & 72.13     & 96.14 \\
        \checkmark & \checkmark     & \textbf{98.27}    & \textbf{94.46}    & \textbf{85.25}    & 72.69     & 97.60 \\
        \bottomrule
    \end{tabular}
    \captionof{table}{Qualitative results on discussing constraints. The top-2 results are in \textbf{bold} and \uline{underline}, respectively.}
\end{minipage}
\hfill
\begin{minipage}[c]{0.29\textwidth}
    \centering
    \includegraphics[width=\linewidth]{asset/ablation.pdf}
    \captionof{figure}{Qualitative results on discussing constraints.}
    \label{fig:ablation}
\end{minipage}

==> table/quan_full_v1.tex <==
\newlength{\umaxwidth}
\settowidth{\umaxwidth}{\(\mathbf{u^{w}}\)}

\centering
% \setlength{\tabcolsep}{4pt}
% \setlength{\extrarowheight}{1pt}
\resizebox{\textwidth}{!}{
    \small
    \begin{tabular}{rcccccccc} 
    \toprule
    {\textbf{Methods}}        
    & \multicolumn{3}{c}{\textbf{Gait Rec. \scriptsize{(CASIA-B)}}}         
    & \multicolumn{2}{c}{\textbf{Action Rec. \scriptsize{(Diving48)}}}
    & \multicolumn{2}{c}{\textbf{Video Gen. \scriptsize{(MHAD)}}}
    \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}  \(\boldsymbol{{\color{gray}{\Psi \left ( {\color{black} \mathbf{u}^{?}}   , \mathbf{v} \right )}}}\)
    & {\small\textbf{NM@R1}\(\uparrow\)}    & {\small\textbf{BG@R1}\(\uparrow\)}    & {\small\textbf{CL@R1}\(\uparrow\)}
    & {\small\textbf{Acc@1}\(\uparrow\)}    & {\small\textbf{Acc@5}\(\uparrow\)}
    & {\small \textbf{SSIM \(\uparrow\)}}   & {\small\textbf{FVD \(\downarrow\)}}
    \\
    \midrule
    Baseline\(^{*}\)    & 92.82     & 82.25     & 69.24     & 65.58     & 95.18     & 0.9463     & 329.22 \\
    \midrule
    RAFT \scriptsize{~\cite{teed2020raft}}                                 & 93.28     & 82.21     & 70.55     & 66.09     & 93.45              & 0.9557            & 118.13 \\
    GMA \scriptsize{~\cite{jiang2021learning}}                             & 93.72     & 83.33     & 71.64     & 69.54     & 94.77              & \uline{0.9565}    & \uline{114.98} \\
    GMFlow \scriptsize{~\cite{xu2022gmflow}}                               & 93.62     & 83.82     & 72.75     & 70.91     & 95.89              & 0.9529            & 429.82 \\
    CRAFT \scriptsize{~\cite{sui2022craft}}                                & 93.71     & 82.89     & 71.12     & 70.20     & 95.74              & 0.9532            & 424.72 \\
    SKFlow \scriptsize{~\cite{sun2022skflow}}                              & 93.52     & 82.38     & 70.53     & 67.26     & 94.57              & 0.9541            & 325.08 \\
    VideoFlow \scriptsize{~\cite{shi2023videoflow}}                        & 93.55     & 82.59     & 70.73     & 71.07     & \uline{96.80}      & 0.9564            & 165.63 \\ 
    FlowFormer\scriptsize{++} \scriptsize{~\cite{shi2023flowformer++}}     & 93.65     & 83.35     & 71.75     & 70.66     & 95.94              & 0.9553            & 284.95 \\ 
    \midrule
    H-MoRe \scriptsize{W.} \small{$\mathmakebox[\umaxwidth][l]{\mathbf{u^{w}}}$}    & 97.13             & 92.31              & 80.78            & 70.91                    & 95.79            & - & - \\
    H-MoRe \scriptsize{L.} \small{$\mathmakebox[\umaxwidth][l]{\mathbf{u^{l}}}$}    & \uline{98.13}     & \textbf{94.91}     & \uline{82.82}    & \textbf{72.74}           & 95.38            & \textbf{0.9574}           & \textbf{108.38} \\
    \midrule
    H-MoRe \scriptsize{W. + L.} \small{$\mathmakebox[\umaxwidth][l]{\mathbf{u^{w+l}}}$}         & \textbf{98.27}             & \uline{94.46}             & \textbf{85.25}             & \uline{72.69} & \textbf{97.60} & - & - \\
    % \midrule
    % SOTA\(^{*}\) & 100.00 & 99.6 & 90.5 & 90.8 & - & - & - \\
    % HuMoR S. + FlowFormer++ & 96.17 & 91.08 & 80.35 \\
    \bottomrule
    \end{tabular}
}

==> table/quan_full_v2.tex <==
\centering
\resizebox{\textwidth}{!}{
    \small
    \begin{tabular}{lcccccccccc} 
    \toprule
    \multirow{2}{*}{\textbf{Methods}}
    & \multicolumn{2}{c}{\textbf{Efficient Analysis}}
    & \multicolumn{3}{c}{\textbf{Gait Rec. \scriptsize{(CASIA-B)}}}         
    & \multicolumn{2}{c}{\textbf{Action Rec. \scriptsize{(Diving48)}}}
    & \multicolumn{2}{c}{\textbf{Video Gen. \scriptsize{(MHAD)}}}
    \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}  
    & {\small\textbf{Params (M)}} & {\small\textbf{FLOPs}}
    & {\small\textbf{NM@R1}\(\uparrow\)}    & {\small\textbf{BG@R1}\(\uparrow\)}    & {\small\textbf{CL@R1}\(\uparrow\)}
    & {\small\textbf{Acc@1}\(\uparrow\)}    & {\small\textbf{Acc@5}\(\uparrow\)}
    & {\small \textbf{SSIM \(\uparrow\)}}   & {\small\textbf{FVD \(\downarrow\)}}
    \\
    \midrule
    \text{w/o Flow} & - & -  & 96.51     & 91.50     & 78.02     & 64.07     & 95.08     & 0.9463     & 329.22 \\
    \midrule
    RAFT \scriptsize{~\cite{teed2020raft}}                                 & 5.258     & 1780.45   & 96.91              & 93.12             & 80.52             & 65.90             & 95.42              & 0.9557               & 118.13 \\
    GMA \scriptsize{~\cite{jiang2021learning}}                             & 5.880     & 2450.31   & 96.61              & 92.83             & 83.63             & 69.00             & 95.62              & \uline{0.9565}       & \uline{114.98} \\
    GMFlow \scriptsize{~\cite{xu2022gmflow}}                               & 4.680     & 428.60    & 97.72              & 93.59             & 85.22             & 71.74             & 95.51              & 0.9529               & 429.82 \\
    CRAFT \scriptsize{~\cite{sui2022craft}}                                & 6.307     & 4204.71   & 96.27              & 92.60             & 79.61             & 71.24             & 95.85              & 0.9532               & 424.72 \\
    SKFlow \scriptsize{~\cite{sun2022skflow}}                              & 6.273     & 2731.59   & 96.59              & 92.42             & 82.13             & 71.39             & 96.64              & 0.9541               & 325.08 \\
    VideoFlow \scriptsize{~\cite{shi2023videoflow}}                        & 12.659    & 3159.37   & \uline{97.88}      & 94.01             & \uline{86.12}     & \uline{72.45}     & \uline{96.72}      & 0.9564               & 165.63 \\ 
    FlowFormer\scriptsize{++} \scriptsize{~\cite{shi2023flowformer++}}     & 16.152    & 3048.14   & 96.66              & \uline{94.31}     & 85.70             & 64.28             & 95.88              & 0.9553               & 284.95 \\ 
    % \midrule
    % H-MoRe \scriptsize{W.} \small{$\mathmakebox[\umaxwidth][l]{\mathbf{u^{w}}}$}    & 97.13             & 92.31              & 80.78            & 70.91                    & 95.79            & - & - \\
    % H-MoRe \scriptsize{L.} \small{$\mathmakebox[\umaxwidth][l]{\mathbf{u^{l}}}$}    & \uline{98.13}     & \textbf{94.91}     & \uline{82.82}    & \textbf{72.74}           & 95.38            & \textbf{0.9574}           & \textbf{108.38} \\
    \midrule
    \methodName{} \scriptsize{Ours}                                        & 5.573    & -    & \textbf{98.26}    & \textbf{95.62}    & \textbf{87.66}    & \textbf{72.99}    & \textbf{97.62} & \textbf{0.9574}    & \textbf{108.38} \\
    % \midrule
    % SOTA\(^{*}\) & 100.00 & 99.6 & 90.5 & 90.8 & - & - & - \\
    % HuMoR S. + FlowFormer++ & 96.17 & 91.08 & 80.35 \\
    \bottomrule
    \end{tabular}
}

==> table/rebuttal_1.tex <==
\begin{table}[h]
  \centering
  \vspace{-8pt}
  \begin{minipage}[t]{0.19\textwidth}
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccc} 
    \toprule
    \(\vartheta_{a}\) & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\)
    \\
    \midrule
    \(5^\circ\)              & 96.31             & 94.12             & 84.98             \\
    \rowcolor{mint}
    \(15^\circ\)             & 98.26             & 95.62             & 87.66             \\
    \(25^\circ\)             & 98.21             & 95.27             & 87.92             \\ 
    \(35^\circ\)             & 97.71             & 94.87             & 85.33             \\ 
    \(45^\circ\)             & 94.80             & 92.20             & 80.19             \\ 
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption{\scriptsize{Angular threshold \(\vartheta_a\).}}
    \label{tab:angular_ablation}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.25\textwidth}
    % \small
    \renewcommand{\arraystretch}{1.67}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccc} 
    \toprule
    Edge Det. & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\)
    \\
    \midrule
    Canny w/o Smoothing              & 97.21             & 95.82             & 87.49             \\
    \rowcolor{mint}
    Canny w/ Smoothing               & 98.26             & 95.62             & 87.66             \\
    EDTER                            & 98.19             & 94.98             & 87.81             \\ 
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption{\scriptsize{Edge detection methods.}}
    \label{tab:boundary_ablation}
  \end{minipage}
  % \caption{Ablation studies for \textbf{\color{darkblue}[R\#P1Zm]}.}
  \vspace{-9pt}
\end{table}


==> table/rebuttal_2.tex <==
\begin{table}[h]
  \centering
  \vspace{-6pt}
  \begin{minipage}[t]{0.18\textwidth}
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccc} 
    \toprule
    Pose Est. & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\)
    \\
    \midrule
    2D Pose {\footnotesize[AlphaPose]}          & 96.82             & 93.44             & 82.17             \\
    \midrule
    H-MoRe {\footnotesize[AlphaPose]}           & 98.04             & 94.22             & 86.91             \\
    H-MoRe {\footnotesize[ViTPose]}             & 98.21             & 94.70             & 87.07             \\
    \rowcolor{mint}
    H-MoRe {\footnotesize[ED-Pose]}             & 98.26             & 95.62             & 87.66             \\
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption*{(a)}
    \label{tab:pose_ablation}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.15\textwidth}
    % \small
    \renewcommand{\arraystretch}{1.48}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccc} 
    \toprule
    Human Seg. & NM@R1\(\uparrow\)    & BG@R1\(\uparrow\)    & CL@R1\(\uparrow\)
    \\
    \midrule
    DINOv2                           & 97.98             & 94.26             & 86.51             \\
    \rowcolor{pink}
    Sapiens                          & 98.34             & 95.71             & 88.10             \\
    \rowcolor{mint}
    U\(^2\)Net                       & 98.26             & 95.62             & 87.66             \\
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption*{(b)}
    \label{tab:segment_ablation}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.12\textwidth}
    \renewcommand{\arraystretch}{1.82}
    \Large
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcc} 
    \toprule
    Models & ACC@1\(\uparrow\) & ACC@5\(\uparrow\)
    \\
    \midrule
    MotionBERT {\footnotesize 3D Pose}                  & 71.51             & 97.09             \\
    MotionBERT {\footnotesize Pretrained Action Rec.}   & 72.32             & 97.71             \\
    \rowcolor{mint}
    \methodName{}                       & 72.99             & 97.62             \\
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption*{(c)}
    \label{tab:pretrained_ablation}
  \end{minipage}
  \vspace{-10pt}
  \caption{Ablation studies on pose estimation and semantic segmentation, as well as comparison with pretrained MotionBERT.}
  \label{tab:rebuttal_2}
  \vspace{-10pt}
\end{table}

% \begin{table}[h]
%     \centering
%     \vspace{-6pt}
%     \resizebox{0.43\textwidth}{!}{
%     \begin{tabular}{lcc} 
%     \toprule
%     Models & ACC@1\(\uparrow\) & ACC@5\(\uparrow\)
%     \\
%     \midrule
%     MotionBERT {\footnotesize 3D Pose}                  & 71.51             & 97.09             \\
%     MotionBERT {\footnotesize Pretrained Action Rec.}   & 72.32             & 97.71             \\
%     \rowcolor{mint}
%     \methodName{}                       & 72.99             & 97.62             \\
%     \bottomrule
%     \end{tabular}}
%     \vspace{-8pt}
%     \caption{\scriptsize{Recognition with pretrained models.}}
%     \label{tab:pretrained_ablation}
%     \vspace{-10pt}
% \end{table}

==> table/rebuttal_3.tex <==
\begin{table}[h]
  \centering
  \vspace{-6pt}
  \begin{minipage}[t]{0.22\textwidth}
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc} 
    \toprule
    Model & CL@R1\(\uparrow\)    & UP@R1\(\uparrow\)    & DN@R1\(\uparrow\)  & BG@R1\(\uparrow\)
    \\
    \midrule
    SMPLGait                                    & 64.2              & 66.8               & 68.1             & 70.2             \\
    \midrule
    SHOF                                        & 72.2              & 75.4               & 74.7             & 77.8             \\
    \rowcolor{mint}
    H-MoRe                                      & 73.8              & 76.7               & 78.3             & 80.2             \\
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption*{(a) Gait Rec. on CCPG}
    \label{tab:pose_ablation}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.24\textwidth}
    % \small
    \renewcommand{\arraystretch}{1.1}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccc} 
    \toprule
    Model. & \(0\)\% & \(0\)\% - \(10\)\% & \(10\)\% - \(20\)\% & \(20\)\% - \(40\)\% & \(40\)\%\(+\)
    \\
    \midrule
    RAFT                          & 69.21             & 65.20             & 61.88             & 58.20             & 48.22             \\
    MHOF                          & 72.94             & 71.66             & 70.31             & 70.77             & 64.79             \\
    \rowcolor{mint}
    \methodName{}                 & 73.42             & 73.09             & 72.68             & 71.62             & 70.81             \\
    \bottomrule
    \end{tabular}}
    \vspace{-8pt}
    \caption*{(b) Action Rec. in Fig.~9}
    \label{tab:segment_ablation}
  \end{minipage}
  \vspace{-10pt}
  \caption{Comparison with SMPLGait, and S/MHOF.}
  \label{tab:rebuttal_3}
  \vspace{-10pt}
\end{table}


==> table/vars_curve.tex <==
\newcommand{\mtmain}[1]{\textbf{#1}}
\newcommand{\mtsub}[1]{\footnotesize{#1}}
\newcommand{\mtcell}[1]{\makecell[lt]{#1}}

\resizebox{0.48\textwidth}{!}{
    \small
    \begin{tabular}{lp{5.4cm}l}
    \toprule
    \textbf{Variables} & \textbf{Description} & \textbf{Type {\footnotesize[shape]}} \\
    \midrule
    \(\boldsymbol{e}\) & Human boundaries. & Curve \\
    \(\boldsymbol{s}\) & Edges of flow map. & Curve \\
    \(\mathcal{P}_{\boldsymbol{e}}\) & Human boundaries within patch \(\mathcal{P}\). & Curve \\
    \(\mathcal{P}_{\boldsymbol{s}}\) & Edges of flow map within patch \(\mathcal{P}\). & Curve \\
    \midrule
    \(p\) & Any point within the human body in the flow maps. & Point \\
    \(\hat{q}\) & The closest point within skeleton offsets \(\vec{\boldsymbol{K}}\) with the highest visibility towards \(p\).  & Point \\
    \(i\) & Any point on the edges of flow map \( \boldsymbol{s} \). & Point \\
    \(\hat{j}\) & The nearest point within human boundaries \(\boldsymbol{e}\) towards \(i\). & Point \\
    \(\boldsymbol{c}_{\mathcal{P}_{\boldsymbol{e}}}\) & The centroid of curve \(\mathcal{P}_{\boldsymbol{e}}\). & Point \\
    \(\boldsymbol{c}_{\mathcal{P}_{\boldsymbol{s}}}\) & The centroid of curve \(\mathcal{P}_{\boldsymbol{s}}\). & Point \\
    \bottomrule
    \end{tabular}
}

==> table/vars_func.tex <==
\newcommand{\mtmain}[1]{\textbf{#1}}
\newcommand{\mtsub}[1]{\footnotesize{#1}}
\newcommand{\mtcell}[1]{\makecell[lt]{#1}}

\resizebox{0.48\textwidth}{!}{
    \small
    \begin{tabular}{lp{5.4cm}l}
    \toprule
    \textbf{Variables} & \textbf{Description} & \textbf{Type {\footnotesize[shape]}} \\
    \midrule
    \(\Phi\) & \mtmain{\methodName{}'s network component.} \mtsub{It estimates world flow \(\boldsymbol{M_w}\) between consecutive frames \(\boldsymbol{X}_{t}\) and \(\boldsymbol{X}_{t+1}\).} & \mtcell{Network \\ {\footnotesize[Params: \(\approx 3.4M\)]}} \\ 
    \(\Psi\) & \mtmain{\methodName{}'s network component.} \mtsub{It estimates subject motion \(\boldsymbol{v_s}\) based on world flow \(\boldsymbol{M_w}\).} & \mtcell{Network \\ {\footnotesize[Params: \(\approx 2.1M\)]}} \\ 
    \midrule
    \(\mathcal{F}\) & \mtmain{Our skeleton constraint.} \mtsub{It ensures that each body point's movement adheres to kinematic constraints.} & Function \\ 
    \(\mathcal{G}\) & \mtmain{Our boundary constraint.} \mtsub{It aligns human shapes onto our estimated flow maps.} & Function \\ 
    \(\mathcal{F_A}\) & \mtmain{Angular constraint.} \mtsub{Component of skeleton constraint.} & Function \\
    \(\mathcal{F_I}\) & \mtmain{Intensity constraint.} \mtsub{Component of skeleton constraint.} & Function \\
    \(\mathcal{C}\) & Chamfer distance between two curves. & Function \\
    \(\mathcal{D}\) & Euclidean distance between two points. & Function \\
    \midrule
    \(\omega_{1}\) & Learnable parameters in \(\Phi\). & Parameters \\
    \(\omega_{2}\) & Learnable parameters in \(\Psi\). & Parameters \\
    \midrule
    \(\vartheta_{a}\) & Threshold for angular constraint \(\mathcal{F}_{A}\). & Constant \\
    \(\vartheta_{i}^{l}\) \(\vartheta_{i}^{h}\) & Low and high boundary threshold for intensity constraint \(\mathcal{F}_{I}\). & Constant \\
    \bottomrule
    \end{tabular}
}

==> table/vars_matric.tex <==
\newcommand{\mtmain}[1]{\textbf{#1}}
\newcommand{\mtsub}[1]{\footnotesize{#1}}
\newcommand{\mtcell}[1]{\makecell[lt]{#1}}

\resizebox{0.48\textwidth}{!}{
    \small
    \begin{tabular}{lp{5.4cm}l}
    \toprule
    \textbf{Variables} & \textbf{Description} & \textbf{Type {\footnotesize[shape]}} \\
    \midrule
    \(\boldsymbol{M_w}\) & \mtmain{\methodName{}'s world flow.} \mtsub{It represents the offset of each body point relative to the environment, \eg, the ground or the camera.} & \mtcell{Matrix \\ {\footnotesize\(\left[ H \times W \times 2 \right]\)}} \\ 
    \(\boldsymbol{M_l}\) & \mtmain{\methodName{}'s local flow.} \mtsub{It represents the offset of each body point relative to the subject themselves.} & \mtcell{Matrix \\ {\footnotesize\(\left[ H \times W \times 2 \right]\)}} \\ 
    \(\boldsymbol{X}_{t}\) \(\boldsymbol{X}_{t+1}\) & \mtmain{Two consecutive frames.} \mtsub{They are usually two frames from a video, spaced more than 0.1 seconds apart.} & \mtcell{Matrix \\ {\footnotesize\(\left[ H \times W \times 3 \right]\)}} \\ 
    \(\boldsymbol{K}_{t}\) \(\boldsymbol{K}_{t+1}\) & \mtmain{Skeleton maps.} \mtsub{They represent a series of (210) skeletal points of a person in frames \(\boldsymbol{X}_{t}\) and \(\boldsymbol{X}_{t+1}\), with each point containing coordinates and visibility information (\(c\)).} & \mtcell{Matrix \\ {\footnotesize\(\left[ 210 \times 3 \right]\)}} \\
    % \(\boldsymbol{K}_{t+1}'\) & \mtmain{Aligned skeleton map.} \mtsub{It calculated by aligning \(\boldsymbol{K}_{t+1}\) to \(\boldsymbol{K}_{t}\).} & \mtcell{Matrix \\ {\footnotesize\(\left[ 210 \times 3 \right]\)}} \\
    \(\vec{\boldsymbol{K}}\) & \mtmain{Skeleton offsets.} \mtsub{It represents the offset of each point in the skeleton map between two time steps, \ie, \(\boldsymbol{K}_{t+1} - \boldsymbol{K}_{t}\)}. & \mtcell{Matrix \\ {\footnotesize\(\left[ 210 \times 3 \right]\)}} \\
    % \(\vec{\boldsymbol{K}}'\) & \mtmain{Skeleton offsets.} \mtsub{It represents the offset of each point in \(\boldsymbol{K}_{t+1}'\) and \(\boldsymbol{K}_{t}\)}. & \mtcell{Matrix \\ {\footnotesize\(\left[ 210 \times 3 \right]\)}} \\
    \midrule
    \(\boldsymbol{v_s}\) & \mtmain{Subject motion.} \mtsub{It represents the overall motion trend of subjects.} & \mtcell{Vector \\ {\footnotesize\(\left[ \Delta x, \Delta y \right]\)}} \\ 
    \(\boldsymbol{u_p}\) & The estimated flow \(\boldsymbol{M}\) at point \(p\). & \mtcell{Vector \\ {\footnotesize\(\left[ \Delta x, \Delta y \right]\)}} \\
    \(\boldsymbol{k_\hat{q}}\) & The skeleton offset \(\vec{\boldsymbol{K}}\) at point \(\hat{q}\). & \mtcell{Vector \\ {\footnotesize\(\left[ \Delta x, \Delta y \right]\)}} \\
    \bottomrule
    \end{tabular}
}
